HiPPO-Prophecy: State-Space Models can Provably Learn Dynamical Systems in Context

This work explores the in-context learning capabilities of State Space Models (SSMs) and presents, to the best of our knowledge, the first theoretical explanation of a possible underlying mechanism. We introduce a novel weight construction for SSMs, enabling them to predict the next state of any dynamical system after observing previous states without parameter fine-tuning. This is accomplished by extending the HiPPO framework to demonstrate that continuous SSMs can approximate the derivative of any input signal. Specifically, we find an explicit weight construction for continuous SSMs and provide an asymptotic error bound on the derivative approximation. The discretization of this continuous SSM subsequently yields a discrete SSM that predicts the next state. Finally, we demonstrate the effectiveness of our parameterization empirically. This work should be an initial step toward understanding how sequence models based on SSMs learn in context.

==> sections_submission_old/abstract.tex <==
This work explores the in-context learning capabilities of State Space Models (SSMs) and, to the best of our knowledge, provides the first theoretical explanation of a potential mechanism underlying them. We introduce a novel weight construction for Linear SSMs, allowing them to predict the next state of any dynamical system after observing previous states, without requiring parameter fine-tuning. To do so, we study Linear SSMs under the HiPPO framework and extend it to show that they are capable of approximating the derivative of the input signal. We then derive an asymptotic error bound on the approximation of this derivative. Discretizing the SSM results in a weight construction that predicts the next state of the dynamical system. Following this, we demonstrate the effectiveness of our parametrization empirically. This work should serve as an initial step towards a better understanding of how neural sequence models based on state space models learn in-context. 


% To do so, we study the Linear State Space Layer (LSSL) under the HiPPO framework and extend it to show that to predict the next state of dynamical systems based on previous observations. We provide explicit weight constructions that lead to the mentioned capability and empirically verify our theory. We hope that this research opens new paths for understanding State Space Models in complex sequence modelling tasks, challenging traditional transformer architectures.
% In this work, we introduce a novel parameter construction for Linear State Space Models, allowing them to predict the next state of any dynamical system after observing previous states, without requiring parameter fine-tuning. This is the first theoretical demonstration that state space models (SSMs) can perform in-context learning (ICL). We extend the HiPPO framework to show that LSSMs can approximate the next state up to first order using an explicit weight construction and provide an asymptotic bound on the approximation error. Our empirical evaluation across various function classes, model sizes, and context lengths demonstrates that our weight construction enables LSSMs to effectively leverage context for accurate predictions, serving as a robust initialization method.

==> sections_submission_old/conclusions.tex <==
\section{Conclusions}
% We succesfully extende on HiPPOs theory framework to enable LSSMs to predict the next step of a dynamical system based on first order approximation. We find both theoretical guarantees and strong emprirical evidence of our construction enabling the model to perform nontrivial next token prediction only based on previously observed signals.
% To the best of our knowledge, this is the first time it was theoretically shown that an SSM can perform autoregressive ICL, although it does not yet account for the few-shot ICL setting.
In this work, we propose a novel LSSM construction that can predict the next state of any dynamical system from its history without fine-tuning its parameters. To the best of our knowledge, this is the first time it was theoretically shown that SSMs can perform autoregressive ICL. We then provide theoretical guarantees for the approximation error of our constructions and analyze their performance on a range of function classes. We find that our weight construction allows LSSMs to effectively leverage context to make predictions and that it can serve as a good initialization.

\section{Broader Impact Statement}
In this work we aim to advance the field of Neural Sequence Modeling and in particular SSMs. Although there might be potential societal consequences of our work, we do not think any of them must be specifically highlighted here



==> sections_submission_old/experiments.tex <==
\section{Experiments}
We perform a thorough experimental evaluation of the weight construction presented in Equation \ref{discretized_sys} and its ability to predict the next value $u_{k+1}$ given its history as context. 
%We provide insight into how our method translates to finite state space dimension ($N < \infty$) and how this width of the model $N$ affects performance.
%Unless otherwise stated we provide the model with the first 5k values of a signal $u$ and afterward unroll the model step-by-step for 5k further steps to predict $u(k+1)$ conditioned on the true signal up to step $k$, $\forall k \in [5001,10000]$. 
For this, we unroll the model step-by-step to predict $u_{k+1}$ by providing it with the true input signal $u_{k}$ for all $k$. We evaluate the model on the second half of the signal to mitigate the errors in the early predictions. This choice is motivated by the analyses depicted in \ref{subfig:time_dependence}, where we find that a sufficiently long previous context length is necessary for the model to predict the next value. The error is taken to be the average absolute distance between the last half of the ground truth signal and the one-step predictions, i.e. \smash{$L=\frac{1}{a}\sum_{k=a}^{2a} |\widehat{u}_{k+1}-u_{k+1}|$}. We refer to Appendix \ref{App: exp} for further details about the experiments.
%= \frac{1}{a}\sum_{k=a}^{2a} |\overline{\C} x_{k+1}+\overline{\D} u_k-u_{k+1}|$. 
%We motivate this choice by drawing the parallel with ICL and analyse the impact of provided context length in Figure \ref{subfig:time_dependence}.
%, as uses data from context to learn a task, here we use the initial points of the signal to let the model stabilize its prediction.\\
\par
\textbf{Ordinary Differential Equation} 
 Motivated by the importance of differential equations in the natural sciences, we compare our model's ability to predict the next state of an adapted  Van der Pol Oscillator in one variable. More specifically, we consider: $\dot{u}(t) = \mu (1-u(t)^2) \sin(t)$. We find that for a hidden state size of $N=65$ both LegT and FouT achieve low error in low-curvature regions. LegT however achieves lower error in high curvature regions which suggests that the model is utilizing the 1st order gradient to predict the next step as proposed by our theory.
\par
\textbf{White Signal and Filtered Noise Process} 
Following \citet{NEURIPS2020_102f0bb6} we use band-limited \ref{subfig:filtered_error} and low pass filtered \ref{subfig:whitenoise_error} white noise, which we refer to as White Signal an Filtered Noise respectively (see Appendix \ref{app:nengo}). For each we use three progressively harder setups in which the high frequency information is increased. For Filtered noise, the frequency content is controlled by $\alpha$, and by $\gamma$ for White Noise. Smaller $\alpha$ and larger $\gamma$ correspond to more high frequency content.
Importantly, we test the model over different hidden state sizes ranging from 1 to 100 in increments of 5. We find that using a larger hidden state dimension is beneficial up to a certain $N$, after which for LegT there is minimal to no further benefit. For FouT on the other hand, the performance gets worse first and then increases again with $N$. This is due to the fact that for low $N$, $\overline{\C}\approx 0, \overline{\D} \approx 1$ and hence the model simply copies its input, which is only outperformed for larger $N$. Note that if the signal is not too discountinuous, copying is a strategy that results in a relatively low error since the current value of the signal and the next are fairly close.\par
% To further investigate this behaviour, we provide an alternative construction for $\overline{\C},\overline{\D}$ in the the FouT basis, which enables us to provide an error bound on the gradient approximation $\dot{u}(t)$. More formally:


% We now pass to validate our construction. First, we show that our weight construction can approximate a range of data from a diverse pool of time series. Please note that we are not fine-tuning our weights to the time series, but we keep the weights frozen and let the model predict the next input given the current one at any time step. This makes our approach valuable as it can be seen as a very simple "Foundation Model" for time series in that it can approximate a very broad range of different time series very well without the need for fine-tuning.\\
% Next, we perform some ablations to show the trend of the performance of our methods as we increase the state dimension $N$. We show that as one would expect, performance improves and the loss decreases as we increase $N$, since we have a better approximation of $\dot{u}(t)$. We also provide a bound that is in accordance with the empirical evidence we observe.\\
% Finally, we will also compare the performance of different initializations of $\A$, $\B$, $\C$ and $\D$. In particular, we train on a Mixed Dataset containing different types of functions (Legendre polymomials, sum of sines and functions sampled from Nengo's WhiteSignal) and then we test on a holdout dataset of previously unseen types of function (Linear, FilteredNoise, the Van der Pool's Oscillator and Bernoulli's equation).

% \subsection{Validation of our weights construction}


% \subsubsection{Nengo Library: WhiteSignal and FIlteredNoise Processes}
% We will first test our weight construction on functions generated via Nengo's WhiteSignal and Filtered Noise functions for validation. The first generates a band-limited white noise process with frequencies below a given cutoff frequency specified by the user. The second one takes a white noise signal and passes it through a filter. Using any type of lowpass filter (e.g., Lowpass, Alpha) will result in a signal similar to WhiteSignal. Still, rather than being ideally filtered (i.e., no frequency content above the cutoff), the FilteredNoise signal will have some frequency content above the cutoff, depending on the filter used. For each of the two, we sample 100 different functions at random and test our SSM for the LegT and FouT construction on all the sampled functions. We report mean and standard deviation of the MSE for the two constructions in Table \ref{nengo}. We compare state dimension $N=33$ and $N=65$ with 10000 data points sampled from the functions. For WhiteSignal, we compare cut-off frequencies $0.3$, $1$ and $2$. Note that as frequency increases, we get more wiggling functions which are harder to approximate (See Figure \ref{fig:fun_approx}. For FilteredNoise, we use the Alpha filter with parameters $0.05$, $0.1$ and $0.3$. Here, as $\alpha$ decreases, we get more rough and wiggling functions which are more difficult to approximate.(See Figure \ref{fig:fun_approx}). Note that we have shifted the ground truth function up by 0.1 to distinguish it from the model's predictions. We note that, in general, the functions generated using the WhiteSignal process are smoother and, hence, easier to approximate. In contrast, the ones generated by FilteredNoise are more rough and discontinuous and, hence, harder to approximate. We indeed note that although the approximation is extremely good in both cases, the model achieves better performance on WhiteNoise as one would expect. We observe that on WhiteSignal with $N=65$, LegT consistently outperforms FouT by at least one order of magnitude, whereas for $N=33$ LegT works better apart from when $\text{freq}=2$. For FilteredNoise instead, both for $N=33$ and $N=65$, FouT performs better for the more difficult scenarios ($\text{alpha} = 0.05$) and ($\text{alpha} = 0.1$) whereas Legt works better for $\text{alpha} = 0.3$.\color{red} Do we want to give some intuitive explanation of why one performs better than the other? Also, do we want to compare performance across different values of $N$ here or we just leave this for experiment 2?\color{black}

%\begin{table}[]
    %\label{nengo}
    %\centering
    %\begin{tabular}{ |p{3cm}||p{3cm}|p{3cm}|p{3cm}|  }
 %\hline
 %\multicolumn{4}{|c|}{Country List} \\
 %\hline
 %& WhiteSignal (freq=1)& Filtered Noise (alpha=0.1)\\
 %\hline
 %LegT \ ($N=17$) & $2.6 \pm  1.4$ \ (1e-6)  &  $2.4 \pm 0.2$ \ (1e-4)\\
% LegS \ ($N=17$)&  $1.2 \pm 0.8$ \ (1e-6)  & $5.2 \pm 3.4$  \ (1e-4)\\
 %FouT \ ($N=17$)& $3.1 \pm 0.9$ \ (1e-6) & $2.3 \pm 0.2$ \ (1e-4)\\
% LegT \ ($N=33$) & $2.2 \pm  1.8$ \ (1e-7)  &  $2.3 \pm 0.2$ \ (1e-4)\\
% LegS \ ($N=33$)&  $2.2 \pm 2.0$ \ (1e-8)  & $6.5 \pm 8.7$  \ (1e-3)\\
% FouT \ ($N=33$)& $3.8 \pm 1.6$ \ (1e-6) & $2.3 \pm 0.2$ \ (1e-4)\\
% LegT \ ($N=65$) & $3.0 \pm  1.1$ \ (1e-7)  &  $2.7 \pm 0.2$ \ (1e-4)\\
% LegS \ ($N=65$)&  $1.1 \pm 1.4$ \ (1e-7)  & $0.2 \pm 0.3$  \\
% FouT \ ($N=65$)& $5.9 \pm 2.3$ \ (1e-6) & $2.4 \pm 0.2$ \ (1e-4)\\

% \hline
%\end{tabular}

    %\caption{Performance of LegT, LegS, and FouT on two Nengo Processes, particularly WhiteSignal and Filtered Noise. The entries represent the MSE of the method with $N=17$}
%\end{table}




%\begin{figure}
    %\centering
    %\includegraphics[width=0.5\linewidth]{function_approx_whitenoise_9.jpg}
    %\caption{Example of one function sampled from a WhiteSignal Process and predictions with $N=17$ and max frequency equal 1 \color{red} TODO: shift predictions so they do not overlap and put more images\color{black}}
    %\label{fig:whitenoise}
%\end{figure}

%\begin{figure}
    %\centering
    %\includegraphics[width=0.5\linewidth]{function_approx_filterednoise_9.jpg}
    %\caption{Example of one function sampled from a FilteredNoise Process and predictions with $N=17$ and alpha equal 0.1 \color{red} TODO: shift predictions so they do not overlap and put more images\color{black}}
   % \label{fig:filterednoise}
%\end{figure}

% \subsubsection{Approximating an ODE}

% Differential equations are the principal tool physicists use to describe and model natural phenomena. We will also validate our approach on differential equations taken from physics, as we think this provides an interesting application of our approach. In particular, we take two very famous differential equations, namely the Bernoulli equation and the Van der Pool oscillator. Note that the second is a second-order differential equation. However, we will show that our method, even though it is originally designed for first-order differential equations, still performs very well.\\
% The Bernoulli equation takes the following form:

% \begin{equation}
%   \frac{dy}{dx}+P(x)y= Q(x) y^n  
% \end{equation}

% In our case, we use $P(x) = \cos(5x)$, $Q(x)=\sin(x)$ and $n=\frac{1}{2}$. We plot the true solution versus the prediction of LegT and FouT in Figure \ref{fig:physics_ode} (where again we shift the true function by 0.1 to avoid overlapping), and we report the performance of the two methods in Table \ref{tab:physic_ode}. Again, we compare performance for state dimension $N=33$ and $N=65$. We notice that for $N=33$, Legt and FouT perform comparably whereas for $N=65$ LegT outperforms FouT.\\
% Here, we adapt the Van der Pool's Oscillator to only one variable, and we add an oscillating component to the equation to make it harder to approximate, leading to:

% \begin{equation}
%     \frac{dy}{dx} = \mu (1-y^2) \sin(x)
% \end{equation}

% where $\mu$ is a hyperparameter. Here, we use $\mu=7$ and $N=17$. We plot the solution and our predictions in Figure \ref{fig:physics_ode} and Table \ref{tab:physic_ode}. We notice that for both $N=33$ and $N=65$ LegT significantly outperforms FouT by at least one order of magnitude. We remark that by looking at Figure \ref{fig:physics_ode}, we can see that it is very similar to a square wave. Note that for this function it is very hard to predict the next value due to the very steep sudden increase/decrease in the y value after a flat region.

% \begin{figure}
    
%     \includegraphics[width=0.5\linewidth]{sections/van_der_pool_N_65.jpg}
%    \hfill
%    \includegraphics[width=0.5\linewidth]{sections/bernoulli_N_65.jpg}
%     \caption{(Left)Solution and Predictions for Van der Pool's Oscillator with $N=65$. (Right) Solution and Prediction for Bernoulli's Differential Equation with $N=65$}
%     \label{fig:physics_ode}
% \end{figure}


%\begin{figure}
    %\centering
    %\includegraphics[width=0.5\linewidth]{van_der_pool.jpg}
    %\caption{Solution and Predictions for Van der Pool's Oscillator}
    %\label{fig:van_der_pool}
%\end{figure}
%\begin{figure}
    %\centering
    %\includegraphics[width=0.5\linewidth]{bernoulli.jpg}
    %\caption{Solution and Prediction for Bernoulli's Differential Equation}
   % \label{fig:bernoulli}
%\end{figure}


% \subsection{Ablations on behavior of predictions for increasing state dimension}

% \color{red} TODO: do we want to use L2 loss instead of L1 to evaluate here? (so that we are consinstent with Experiment 2) \color{black}
% In this section, we aim to validate the intuition that if we increase the state dimension $N$, the performance of our parametrization also increases. This is simply because as we have shown in the two different parametrizations of Hippo-LegT and FouT, we can express $\dot{u}$ as an infinite series of terms of which we are only taking a finite amount $N$. As $N$ increases, we are simply considering more and more terms of the series and hence we expect our approximation to be better. For this ablation, we take the WhiteSignal and FilteredNoise with $\text{freq}=1$ and $\text{alpha}=0.1$ respectively and we let $N$ vary from \color{red} TODO: decide \color{black} to \color{red} TODO \color{black}. For both WhiteSignal and FilteredNoise, we plot in the same Figure
% .
\textbf{Learning from Context}
To provide empirical evidence of our models utilizing their context we investigate their performance dependent on the number of previous signal points they have seen in context. Overall, in \ref{subfig:time_dependence} we find that for all $N$ the model gets better with larger context effectively increasing its accuracy by leveraging information from its context. We find that for more expressive models with larger hidden states, oscillations happen for longer and thus require more samples to stabilize. This is to be expected as larger values of $N$ correspond to bigger function classes that the model can represent.
% In order to do so, we will look at a slightly different way to derive an approximation of $\dot{u}(t)$ and to derive the parametrizations for $\C$ and $\D$ than the ones we presented above that will make the analysis more accessible. Starting from Equation \ref{reconstruction}, we have the following:

% \begin{equation}
%     \dot{u}(s) = \sum_{n=0}^{\infty} x_n(t) \frac{\partial}{\partial s}p_n(t,s) \ \ \forall s < t
% \end{equation}

% Note that by assuming continuity of $\dot{u}$ and $p_n$ w.r.t. $s$, we can take the limit from the left as $s$ goes to $t$, giving us:

% \begin{equation}
%     \dot{u}(t) = \sum_{n=0}^{\infty} x_n(t) \frac{\partial}{\partial s}p_n(t,s) \Big |_{s=t} 
% \end{equation}

% We focus the analysis using the FouT parametrization for $\A$ and $\B$. We then have the following result for construction of $\C$ and $\D$ for FouT:

% \begin{restatable}[Alternative FouT construction]{prop}{FouTAlt}
% \label{fout_alt}
% If we choose $\C_k = \begin{cases}
%         0 & \text{if} \: k=0 \text{ or } k \text{ odd}\\
%         -2 \sqrt{2}\pi n & \text{otherwise} \quad
%     \end{cases}$ \ \ \ and $
%     \D = 0$ and $\A$, $\B$ and $p_k(t,s)$ as in HiPPO FouT, then the output $y(t)$ is an approximation of $\dot{u}(t)$ based on $N$ basis functions.
% \end{restatable}


% Given the above construction, we now want to find a bound on the approximation error we make by truncating the expansion of $\dot{u}(t)$ up to N terms. We denote this approximation $\dot{u}_N(t)$. From this, We also derive an approximation bound on $\widehat{u}_N(t)$, where $\widehat{u}_N(t) = \int_{0}^t \dot{u}_N(s) ds$ is the approximation of $u(t)$ by integrating the truncated version of its time derivative. This reflects the way we derive an estimate of the next step of $u$ in this work. Please note that we do not consider the error coming from the discretization in this work for simplicity of explanation and leave this to future work. We have the following results:

% \begin{restatable}[Local Approximation Error]{thm}{ApproxErr}
% \label{approx_error}
%     If $u$ has k-th bounded derivatives for some $k \geq 3$, i.e. $|u^{(k)}(t)| \leq L \ \forall t$, then it holds that for the choice of $\A$ and $\B$ in Hippo FouT and $\C$ and $\D$ as in Prop. \ref{fout_alt}:
%     \begin{equation*}
%         \left|\dot{u}(t) - \dot{u}_N(t)\right| \in \mathcal{O}\left(\frac{L}{N^{k-2}}\right)
%     \end{equation*}
% \end{restatable}

% As a corollary of the above, we get that:

% \begin{restatable}[Approximation Error]{cor}{ApproxErrCor}
% \label{cor:ApproxErrCor}
%     Under the same assumptions and parametrization as in Theorem \ref{approx_error}, we have that:

%      \begin{equation*}
%          \left|u(t) - \widehat{u}_N(t)\right| \in \mathcal{O}\left(\frac{Lt}{N^{k-2}}\right)
%       \end{equation*}
    
% \end{restatable}

% As we remarked above, the bound above holds for continuous time and not for the discrete time counterpart. When trying to implement the above construction in discrete time, we noticed that it is more unstable than the other two constructions and hence we decided to stick with them in the experiments. \color{red} Do we want to say more about this here? \color{black}

\input{sections/main_figure}

\textbf{Constructions as Initialisation}
In \ref{subfig:construction_vs_training} we compare the the performance of LSSM layers in different settings. $(\mathrm{I})$ Initializing $\overline{\A},\overline{\B},\overline{\C},\overline{\D}$ at construction and training $\overline{\C},\overline{\D}$. $(\mathrm{II})$ Our weight construction. $(\mathrm{III})$ Initializing $\overline{\A},\overline{\B}$ at construction, standard Gaussian initialization and training of $\overline{\C},\overline{\D}$. $(\mathrm{IV})$ Initializing $\overline{\A},\overline{\B},\overline{\C},\overline{\D}$ at construction and training all of them. We train the models on a mixed dataset, consisting of a mixture of different function classes as outlined in Appendix \ref{subsec:experiment3}. We evaluate all these models on 3 hold out datasets, namely filtered noise,  a holdout mixed dataset and linear functions and Van der Pol's signal (which is also holdout), given in \ref{subfig:van_der_pol}. We observe that our parametrization $(\mathrm{II})$ is competitive with trained SSMs.
%In \ref{subfig:construction_vs_training} we show that for training a single Linear State Space Model, initializing the model with our weight constructions, leads to significantly better performance on next value prediction than training from random initialization. Even initialization  $A, B$ to the HiPPO-LegT matrices performs significantly worse than setting $C, D$ to our proposed constructions. The models were trained on 3 different random seeds each and bot avg, min, and max bounds are plotted. For a detailed description of the experiment consider Appendix \ref{App: exp}.


% In these experiments, we aim to show that when training on a diverse range of functions and want to test generalization of the model, i.e. testing on a holdout dataset of unseen function types, the best performing model is the one initialized with our parametrization. For this ablation, we will use the LegT parametrization with $N=32$. More precisely, we compare three different types of initializations, namely initializing all of $\A$, $\B$, $\C$ and $\D$ following our parametrization, initializing $\A$ and $\B$ as in LegT and then $\C$ and $\D$ at random and then initializing all the four matrices at random. We will also compare these three with our parametrization with fixed parameters (i.e. we do not train on the training dataset but we only evaluate on the hold out dataset). We observe that \color{red} TODO: complete observations once we have results from all the seeds \color{black}.


==> sections_submission_old/introduction.tex <==
\section{Introduction}
In-context learning (ICL) refers to a model's ability to solve tasks, unseen during training, only based on information provided in-context, without updating its weights. ICL has gained significant attention since \citet{brown2020language} demonstrated that transformer models \cite{vaswani2023attention} trained on large and diverse language corpora can learn in-context without being explicitly trained for it. More specifically, they showed that given a sequence of input-output pairs from an unseen task, the model is capable of predicting the output corresponding to a new input. We will refer to this type of ICL as few-shot in-context learning, to emphasize the presence of input-output pairs in-context\footnote{Prior to \cite{brown2020language}, ICL was only observed in the few-shot learning setting (without weight updates), where models were explicitly trained to infer the output corresponding to an input when provided with example input-output pairs from an unseen task \cite{vinyals2017matching, santoro2016oneshot}.}. %An example of few-shot ICL is that of regression where the model is provided with $(x_i, f(x_i))_{i\leq n}$ and is tasked to predict $f(x')$ given a query point $x'$.
Subsequently to \cite{brown2020language}, there have been a variety of empirical \cite{olsson2022incontext, kossen2024incontext, wei2023larger, garg2023transformers} as well as theoretical \cite{vonoswald2023transformers, akyürek2023learning, bai2023transformers, vladymyrov2024linear,zhang2023trained,wu2024pretraining, zhang2024incontext,mahankali2023step, ahn2023transformers} works studying the few-shot ICL capabilities of transformer models and the mechanisms underlying them. In addition to the few-shot ICL setting, there have been a number of papers investigating how in-context learning arises when the models are trained autoregressively on sequential data \cite{akyürek2024incontext, vonoswald2023uncovering}, the primary training mode of sequence models. We label this mode as autoregressive ICL.
An example would be predicting the next value \smash{$f(x_{t})$} of an out-of-distribution time series given previous values $\{f(x_i)\}_{i < t}$ in-context.
\par
Concurrently to these studies, the development of deep state space models such as S4 by \citet{gu2022efficiently} has sparked a resurgence of recurrent sequence models, resulting in a family of models, which we will refer to as  generalized state space models (GSSMs) \cite{hasani2022liquid,gu2022parameterization, orvieto2023resurrecting, fu2023hungry,gu2023mamba, de2024griffin}. GSSMs offer a promising alternative to transformers by addressing two fundamental challenges, namely length generalization and quadratic computational cost (flops) with respect to the sequence length \cite{gu2023mamba}. 
%GSSMs overcome these limitations by not relying on the all-to-all attention computation between inputs but rather computing the sequence recurrently, with linear cost. Unlike nonlinear RNNs \cite{} the computation of GSSMs is fully parallelizable thanks to their linear recurrence. 
Similarly to transformer-based models, GSSMs have empirically been shown to be capable of ICL \cite{lu2023structured, akyürek2024incontext, park2024mamba, grazzi2024mamba}. Nonetheless, our theoretical understanding of the mechanisms underlying ICL in GSSMs is still limited. In this work, to the best of our knowledge, we provide the first explanation of how GSSMs do autoregressive ICL. For this we consider the Linear State Space Layer (LSSL) on the task of predicting the next state of any dynamical system, given a sequence of previous states. Our contributions can be summarized as:
\begin{itemize}[leftmargin=*,itemsep=-3pt]
  \item Extending the HiPPO framework to show that LSSMs can approximate the next state of any dynamical system up to first order, from a sequence of previous states through an explicit weight construction.
  \item An asymptotic bound on the approximation error for continuous LSSMs for the weight construction w.r.t the HiPPO FouT basis.
  \item An experimental evaluation of our weight construction on different function classes, model sizes and context lengths.
\end{itemize}


% \begin{itemize}
%   \item We extend the HiPPO framework to show that LSSMs are capable of approximating the next state of a dynamical system, from a sequence of previous states, by providing an explicit weight construction.
%   \item In the case of continuous LSSMs and the HiPPO-FouT Basis, we provide an asymptotic bound on the approximation error.
%   % For the HiPPO-FouT Basis in the continuous setting we provide an asymptotic bound on the error.
%   \item We provide empirical evidence that our weight construction leads to predictions of the next state of the dynamical system that is competitive with LSSMs after training.
%   % We provide empirical evidence that our general construction of C and D for the FouT and LegT Bases leads to non-trivial prediction of the next signal $u(t+1)$ given sufficient previous observations $u(1:t)$ in context.
%   % Based only on the provided context and using the same weights ($A,B,C,D$) the model can generalize its next value prediction to a diverse set of signals.
% \end{itemize}







% Specifically, \citet{park2024mamba} and \citet{grazzi2024mamba} demonstrate that in simple in-context function approximation tasks, Mamba \cite{gu2023mamba} performs comparably to transformers. 
% Further, \citet{grazzi2024mamba} found that Mamba excels in sparse parity learning but falls short in tasks that require retrieval. The underperformance of GSSMs in retrieval tasks, as compared to transformers, was also confirmed in \cite{akyürek2023learning, jelassi2024repeat}. 

% Although, it has been shown empirically, that GSSMs are capbable of in-context learning, our theoretical understanding of how this happens is still limited. 



%In this work, we aim to bridge this gap by providing the first explanation of how recurrent models based on structured state space models can learn dynamical systems in context.  {\color{red} to be completed once we have our exact contributions}


% and studying them with Bayesian theory \cite{xie2022explanation,wies2023learnability,jeon2024informationtheoretic}.\par



% Large Neural Sequence Models are capable of solving tasks  they were not explicitly trained for, only based on information provided in context without updating their parameters. These capabilities were first showcased by  \citet{brown2020language}, who demonstrated that auto-regressive transformer models trained on large and diverse language corpora \cite{vaswani2023attention} excel at zero-shot generalization and few-shot learning. Zero-shot generalization refers to the models ability to solve unseen tasks when provided with a problem description. Few-shot learning on the other hand is a model's ability to solve a task when provided with input-output pairs without parameter updates \footnote{Traditionally, few-shot learning }.


% These capabilities were first studied in zero-shot and few-shot learning settings, where neural networks were trained to adjust their predictions based on a few examples without weight updates \cite{vinyals2017matching, santoro2016oneshot}. 

% More recently, \citet{brown2020language} demonstrated that auto-regressive transformer models trained on large and diverse language corpora \cite{vaswani2023attention} excel at zero-shot and few-shot generalization, provided with a task description and task examples as context respectively.

% The later setup (few-shot) has become known as In Context Learning which has sparked a variety of general empirical \cite{kirsch2024generalpurpose, olsson2022incontext, kossen2024incontext, wei2023larger, garg2023transformers, akyürek2023learning} studies, as well as theoretical works investigating transformers on regression problems \cite{vonoswald2023transformers, vonoswald2023uncovering, bai2023transformers, vladymyrov2024linear,zhang2023trained,wu2024pretraining, zhang2024incontext,mahankali2023step, ahn2023transformers} and studying them with Bayesian theory \cite{xie2022explanation,wies2023learnability,jeon2024informationtheoretic}.


% Concurrently, the development of deep state space models such as S4 by \citet{gu2022efficiently} has sparked a resurgence of recurrent sequence models, resulting in a family of models which we will refer to as generalized state space models (GSSMs) \cite{hasani2022liquid,gu2022parameterization, orvieto2023resurrecting, fu2023hungry,gu2023mamba, de2024griffin}.


















% Large Neural Sequence Models possess the capability to solve tasks that they were not explicitly trained for, only based on information provided in context without updating their parameters.
% These capabilities were first studied in zero-shot and few-shot learning settings, where neural networks were trained to adjust their predictions based on a few examples without weight updates \cite{vinyals2017matching, santoro2016oneshot}. More recently, \citet{brown2020language} demonstrated that auto-regressive transformer models trained on large and diverse language corpora \cite{vaswani2023attention} excel at zero-shot and few-shot generalization, provided with a task description and task examples as context respectively. The later setup (few-shot) has become known as In Context Learning which has sparked a variety of general empirical \cite{kirsch2024generalpurpose, olsson2022incontext, kossen2024incontext, wei2023larger, garg2023transformers, akyürek2023learning} studies, as well as theoretical works investigating transformers on regression problems \cite{vonoswald2023transformers, vonoswald2023uncovering, bai2023transformers, vladymyrov2024linear,zhang2023trained,wu2024pretraining, zhang2024incontext,mahankali2023step, ahn2023transformers} and studying them with Bayesian theory \cite{xie2022explanation,wies2023learnability,jeon2024informationtheoretic}.
% Concurrently, the development of deep state space models such as S4 by \citet{gu2022efficiently} has sparked a resurgence of recurrent sequence models, resulting in a family of models which we will refer to as generalized state space models (GSSMs) \cite{hasani2022liquid,gu2022parameterization, orvieto2023resurrecting, fu2023hungry,gu2023mamba, de2024griffin}.
%GSSMs offer a promising alternative to transformers by addressing two fundamental challenges; length generalization and quadratic computational cost (flops) with respect to the sequence length \cite{gu2023mamba}.
% %GSSMs offer a promising alternative to transformers by overcoming two fundamental limitations; they can only model sequences inside a finite window and scale quadratically with respect to the sequence length \cite{gu2023mamba}. 
% %GSSMs overcome these limitations by not relying on the all-to-all attention computation $O(N^2)$ between inputs but rather computing the sequence in linear recurrence $O(N)$.
%GSSMs overcome these limitations by not relying on the all-to-all attention computation between inputs but rather computing the sequence recurrently, with linear cost. Unlike nonlinear RNNs \cite{} the computation of GSSMs is fully parallelizable thanks to their linear recurrence.
%Similarly to transformer-based models, GSSMs have empirically been shown to be capable of In Context Learning \cite{lu2023structured, akyürek2024incontext, park2024mamba, grazzi2024mamba, lu2023structured}. Specifically, \citet{park2024mamba} and \citet{grazzi2024mamba} demonstrate that in simple in-context function approximation tasks, Mamba \cite{gu2023mamba} performs comparably to transformers.
%Although it is empirically seen that GSSMs can learn in context, the theoretical understanding of how this happens is still missing.\\

% The first proposed form of these GSSM is the Linear State Space Layer (LSSM) \cite{gu2021combining}, which is a 1-dimensional linear sequence model mapping and input sequence $u(t)$ to an output sequence $y(t)$ via an implicit state $x(t)$. Following their initial success, \citet{gu2022train} presented the HiPPO theory framework studying the expressiveness of SSMs based on their ability to compress information over the history $u(1,2,...,t)$ in its state $x(t)$. They provide evidence of this by showing that their models can recover a previously observed signal only from its current state $x(t)$.
% %and prove that it does so by representing the signal as convolutional kernels provided as linear combinations (defined by C) of basis functions parameterized by A \& B.
% \\ In this work, we provide to the best of our knowledge the first insight into how GSSMs could learn from context by extending the HiPPO framework from its original memorization task to predicting the next value of a signal.
% We consider the Linear State Space Layer (LSSL) on the synthetic task of predicting the next value of a first-order dynamical system.
% Note that this setup moves from the few-shot setting considered by \citet{brown2020language} to the setting of \citet{vonoswald2023uncovering}, which analyses the In-Context-Learning capabilities of Linear Attention as auto-regressive next-value prediction of a sequence. This setup is closely related to predicting the next token in a language modeling task. However, differently from the classical ICL setting, here we do not provide input-label pairs but only previous values of the signal $u$.\\
% Our contributions are summarized as:
% \begin{itemize}
%   \item We extend the HiPPO framework to approximate the next value of any first-order dynamical system: $y(t)=u(t+1)$ given sufficient past observations of the signal. For this, we provide explicit constructions of $C$ and $D$ for HiPPO's FouT and LegT realizations of $A$ and $B$.
%   \item For the HiPPO-FouT Basis in the continuous setting we provide an asymptotic bound on the error.
%   \item We provide empirical evidence that our general construction of C and D for the FouT and LegT Bases leads to non-trivial prediction of the next signal $u(t+1)$ given sufficient previous observations $u(1:t)$ in context.
%   Based only on the provided context and using the same weights ($A,B,C,D$) the model can generalize its next value prediction to a diverse set of signals.

% \end{itemize}














% In-context learning (ICL) refers to a model's ability to solve tasks that it was not explicitly trained for, only based on information provided in context without updating its weights.
% %(e.g. predicting $f(x')$ for an input $x'$ given pairs \smash{$\big(x,f(x)\big)$} in-context).
%These capabilities were first incentivized in few-shot learning settings, where neural networks were trained to adjust their predictions based on a few examples without weight updates \cite{vinyals2017matching, santoro2016oneshot}. More recently, \citet{brown2020language} demonstrated that auto-regressive transformer models trained on large and diverse language corpora \cite{vaswani2023attention} can learn in-context without being explicitly trained for it. This has sparked an increasing academic interest in understanding the ICL capabilities of transformer-based models and the mechanisms underlying them. 
%{\color{red} To this end, there have been a variety of general empirical \cite{kirsch2024generalpurpose, olsson2022incontext, kossen2024incontext, wei2023larger, garg2023transformers, akyürek2023learning} studies, as well as theoretical works investigating transformers on regression problems \cite{vonoswald2023transformers, vonoswald2023uncovering, bai2023transformers, vladymyrov2024linear,zhang2023trained,wu2024pretraining, zhang2024incontext,mahankali2023step, ahn2023transformers} and studying them with Bayesian theory \cite{xie2022explanation,wies2023learnability,jeon2024informationtheoretic}. On the theoretical side, it was shown that in basic supervised learning tasks, such as regression, transformers perform mesa-optimization based on gradient methods to learn in-context.}\par
% Concurrently, the development of deep state space models such as S4 by \citet{gu2022efficiently} has sparked a resurgence of recurrent sequence models, resulting in a family of models which we will refer to as generalized state space models (GSSMs) \cite{hasani2022liquid,gu2022parameterization, orvieto2023resurrecting, fu2023hungry,gu2023mamba, de2024griffin}. 
%GSSMs offer a promising alternative to transformers by addressing two fundamental challenges; length generalization and quadratic computational cost (flops) with respect to the sequence length \cite{gu2023mamba}.
%GSSMs offer a promising alternative to transformers by overcoming two fundamental limitations; they can only model sequences inside a finite window and scale quadratically with respect to the sequence length \cite{gu2023mamba}. 
%GSSMs overcome these limitations by not relying on the all-to-all attention computation $O(N^2)$ between inputs but rather computing the sequence in linear recurrence $O(N)$.
%GSSMs overcome these limitations by not relying on the all-to-all attention computation between inputs but rather computing the sequence recurrently, with linear cost. Unlike nonlinear RNNs \cite{} the computation of GSSMs is fully parallelizable thanks to their linear recurrence. Similarly to transformer-based models, GSSMs have empirically been shown to be capable of ICL \cite{lu2023structured, akyürek2024incontext, park2024mamba, grazzi2024mamba, lu2023structured}. Specifically, \citet{park2024mamba} and \citet{grazzi2024mamba} demonstrate that in simple in-context function approximation tasks, Mamba \cite{gu2023mamba} performs comparably to transformers. 
%Further, \citet{grazzi2024mamba} found that Mamba excels in sparse parity learning but falls short in tasks that require retrieval. The underperformance of GSSMs in retrieval tasks, as compared to transformers, was also confirmed in \cite{akyürek2023learning, jelassi2024repeat}. Although, it has been shown empirically, that GSSMs are capbable of in-context learning, our theoretical understanding of how this happens is still limited. In this work, we aim to bridge this gap by providing the first explanation of how recurrent models based on structured state space models can learn dynamical systems in context.  {\color{red} to be completed once we have our exact contributions}

%Nonetheless, the capabilities of GSSMs to learn in-context remain rather underexplored compared to transformer-based models. \caglar{It is empirically known that SSMs can learn in-context. We have shown several results on this in the Griffin paper. So I would phrase it something like, although it is known that SSMs can learn in-context empirically, the theoretical understanding of how this happens has been missing.} Especially on the theoretical side, there is limited understanding of the mechanisms underlying ICL in GSSMs. 


%Besides these empirical comparisons of the ICL capabilities transformer-based models and GSSMs, our understanding of the mechanisms underlying ICL in GSSMs remains limited. 







%In-context learning (ICL) refers to the ability of a model to solve tasks that it was not explicitly trained for based on information provided in its context and without weight updates.

%In-context learning (ICL) has emerged as a remarkable capability of large neural sequence models, enabling them to accurately predict outputs for new inputs when provided with a sequence of input-output pairs  from an unseen task in-context \cite{brown2020language}. This requires the models to learn a predictor from the provided examples without updating its weights and hence marks a departure from traditional in-weights learning \cite{akyürek2023learning, grazzi2024mamba}. In particular for transformer based architectures \cite{vaswani2023attention}, ICL has gained significant attention from the academic community to better understand it's underlying mechanisms empirically \cite{} and theoretically \cite{}. From a theoretical perspective, research has demonstrated that in basic supervised learning tasks, such as regression, transformers perform mesa-optimization based on gradient methods to learn in-context \cite{}.

% enabling them to accurately predict outputs for new inputs when provided with a sequence of input-output pairs  from an unseen task in-context \cite{brown2020language}.

%This requires the models to learn a predictor from the provided examples without updating its weights and hence marks a departure from traditional in-weights learning \cite{akyürek2023learning, grazzi2024mamba}.

% In-context learning (ICL) has emerged as a fascinating capability of large neural sequence models, where, provided with a set of input-output pairs, the model accurately predicts the output corresponding to a new input. 

 % accurately predict outputs for new inputs on unfamiliar tasks using a set of example input-output pairs.


% \color{blue}
% Things to cover here
% \begin{itemize}
%     \item Start with ICL in general: what is ICL, finding that transformers can do ICL, relevance and power of ICL
%     \item Talk about the observations that have been made in transformers, theoretical and empirical side
%     \item Orthogonally to this, there have been advances in SSMs (S4, S5, H3, Mamba) which perform well on a variety of tasks
%     \item Point to the appendix for a more detailed related works section. (is required?)
%     \item  There have only been empirical findings on the ICL capabilities of SSMs
%     \item To the best of our knowledge, the first theoretical analysis of ICL for SSMs (analogous to say linear regression in transformers)
% \end{itemize}
% \color{black}

==> sections_submission_old/main.tex <==
%\section{Main}
%State space models (SSM) take the following form:

%\begin{equation}
    %\begin{cases}
        %\dot{x}(t) = \A x(t)+\B u(t) \\
        %y(t) = \C x(t)+\D u(t)
    %\end{cases}
%\end{equation}

%In our setting, we consider $u(t) \in \mathbb{R}$ and $x(t) \in \mathbb{R}^N$. It was proven in \citep{NEURIPS2020_102f0bb6} and \citep{gu2022train} that by choosing the matrices $\A$ and $\B$ according to the HIPPO theory, then the hidden state $x(t)$ can be seen to represent an orthogonal projection of the input signal $u_{\leq t}$ onto the $N$-dimensional space of Lagrange polynomials. In particular, in the limit of $N \rightarrow \infty $ we have that:

%\begin{equation}
    %u(s) = \sum_{n=0}^{\infty} x_n(t) p_n(t,s) \ \ \forall s\leq t
%\end{equation}

%with $p_n(t,s)$ being the orthonormal basis. In particular, they consider two settings, namely Hippo-LegT and Hippo-LegS, based on Legendre polynomials, but the first leads to a time-invariant LTI, whereas the second leads to a time-variant system. From above, we easily get that:

%\begin{equation}
%\label{u_t_decomp}
    %u(t) = \sum_{n=0}^{\infty} x_n(t) p_n(t,t) 
%\end{equation}

%The idea behind this construction in \citep{NEURIPS2020_102f0bb6} and \citep{gu2022train} is that $x(t)$ can (approximately) retain all the information up until time $t$ and hence we can approximately reconstruct the input signal up until the current time by using $x(t)$. In this work, we want to take this construction a step further, and in particular, we want to leverage the HiPPO theory to also approximate any first-order dynamical system. In particular, we will show how to construct a parametrization of $\C$ and $\D$ such that $y(t)=\dot{u}(t)$ (in the limit of $N \rightarrow \infty$). 
%To do so, we start from Equation \ref{u_t_decomp} and differentiate $u(t)$ by differentiating the series term by term. We will assume for now that $u(t)$ satisfies the smoothness assumptions required to exchange series and derivative, and we will specify the specific assumptions that $u(t)$ needs to satisfy later. \color{red} TODO: write down formal assumptions in the Propositions\color{black}. Note that also in both LegT and LegS $p_n(t,t)$ is a constant \color{red} TODO: maybe write down explicitly what $p_n(t,s)$ looks like in the two cases \color{black}. Then, we have the following:

%\begin{equation}
%\label{u_t_decomp}
    %\dot{u}(t) = \sum_{n=0}^{\infty} \dot{x}_n(t) p_n(t,t) 
%\end{equation}

%We will now derive the parametrizations for $\C$ and $\D$ for both LegT and LegS, starting from the above equation. We have the following two results:
%\begin{restatable}[LegT construction]{prop}{LegT}
    %\label{prop:LegT}
    %If we choose $\C_j = \sum_{k = 0}^N\A_{kj}p_k(t, t)$ and $
    %\D = \sum_{k = 0}^N \B_k p_k(t, t)$ and $\A$, $\B$ and $p_k(t,t)$ as in HiPPO LegT, then the output $y(t)$ is an $N$-dimensional approximation of $\dot{u}(t)$.
%\end{restatable}
%\vspace{-0.3cm}
%\begin{restatable}[LegS construction]{prop}{LegS}
    %\label{prop:LegS}
    %If we choose $\C_j = \sum_{k = 0}^N\frac{1}{t}\A_{kj}p_k(t, t)$ and $
    %\D = \sum_{k = 0}^N \frac{1}{t}\B_k p_k(t, t)$ and $\A$, $\B$ and $p_k(t,t)$ as in HiPPO LegS, then the output $y(t)$ is an $N$-dimensional approximation of $\dot{u}(t)$.
%\end{restatable}
%Note that to predict the next time-step $u(t+\Delta t)$, we need to approximate the following integral, having access to $u(t)$:
%\begin{equation}
    %u(t+\Delta t) = u(t) +\int_{t}^{t+\Delta t}\dot{u}(s) ds
%\end{equation}

%Since we cannot solve the integral in closed form, we will use discretization, and in particular, the bilinear (also called trapezoid) method, which leads to the following approximation (more details in the Appendix): \color{red} TODO: change into index notation instead of time notation \color{black}

%\begin{align}
    %u(t+ \Delta t) 
    %&\approx \left( 1 - \frac{\D \Delta t}{2}\right)^{-1} \left[ \left( 1 + \frac{\D \Delta t}{2}\right)u(t) + \Delta t \C x(t) \right]\\
   % &= \overline{\C} x(t)+ \overline{\D} u(t)
%\end{align}

%where $C$ and $D$ are the parametrizations of HiPPo LegT and LegS (the discretization leads to the same expression for both methods).\\

%We now propose a different way to calculate $\dot{u}(t)$, which we will base our theoretical analysis on. In particular, instead of first evaluating $u(s)$ at $t$ and then taking the derivative, we will first derive $u(s)$ and only then evaluate the function at $t$. The other difference is that here, we will use the classic Fourier basis of sines and cosines to make the analysis easier. In particular, we have the following:

%\begin{equation}
    %\dot{u}(s) = \sum_{n=0}^{\infty} x_n(t) \frac{\partial}{\partial s}p_n(t,s) \ \ \forall s < t
%\end{equation}

%Note that by assuming continuity of $\dot{u}$ and $p_n$ wrt $s$, we can take the limit from the left as $s$ goes to $t$, giving us:

%\begin{equation}
    %\dot{u}(t) = \sum_{n=0}^{\infty} x_n(t) \frac{\partial}{\partial s}p_n(t,s) \Big |_{s=t} 
%\end{equation}

%HiPPo-FouT assumes $\{p_n\}_{n \geq 0}(t,s) = \sqrt{2} \Big [1 \ \cos(2\pi (t-s)) \ \sin(2\pi (t-s)) \ \cos(4\pi (t-s)) \ \sin(4\pi (t-s)) \ \dots \Big]$ and $\omega(s,t)= \mathbb{1}_{[t-1, t]}(s)$. We now have the following construction of $\C$ and $\D$ for the Fourier basis.

%\begin{restatable}[FouT construction]{prop}{FouT}
%\label{fout}
%If we choose $\C_k = \begin{cases}
        %0 & \text{if} \: k=0 \text{ or } k \text{ odd}\\
       % -2\sqrt{2}\pi n & \text{otherwise} \quad
    %\end{cases}$ \ \ \ and $
    %\D = 0$ and $\A$, $\B$ and $p_k(t,s)$ as in HiPPO FouT, then the output $y(t)$ is an $N$-dimensional approximation of $\dot{u}(t)$.
%\end{restatable}

%In this case, note that we then have $\dot{u}(t) = Cx(t)$. For discretization, we will here use the simpler Euler method instead as it proves sufficiently stable for our purposes:

%\begin{equation}
    %u(t+\Delta t)-u(t) = \int_t^{t+\Delta t} \dot{u}(s) ds \approx \Delta t \dot{u}(t) = \Delta t C x(t)
%\end{equation}

%Hence we have $u(t+\Delta t) = \Delta t C x(t) + u(t)$, which leads to the choice $\overline{C} = \Delta t \ C$ and $\overline{D} = 1$.

%\subsection{Theoretical Analysis}

%Given the above construction, we now want to find a bound on the approximation error that we make by truncating the expansion of $\dot{u}(t)$ up to N terms. We will denote this approximation $\dot{u}_N(t)$. From this, We will also derive an approximation bound on $\widehat{u}_N(t)$, where $\widehat{u}_N(t) = \int_{0}^t \dot{u}_N(s) ds$ is the approximation of $u(t)$ by integrating the truncated version of its time derivative. This reflects the way we derive an estimate of the next step of $u$ in this work. Please note that we will not consider the error coming from the discretization in this work for simplicity of explanation and leave this to future work. Let us note that we will also focus on the FouT parametrization in this work. We will leave the analysis of LegT for future work. We have the following results:

%\begin{restatable}[Local Approximation Error]{thm}{ApproxErr}
%\label{approx_error}
    %If $u$ has k-th bounded derivatives with $k \geq 3$, i.e. $u^{(k)}(t) \leq L \ \forall t$, then it holds that for the choice of $\A$ and $\B$ in Hippo FouT and $\C$ and $\D$ as in Prop. \ref{fout}:

    %\begin{equation*}
        %\left|\dot{u}(t) - \dot{u}_N(t)\right| \in \mathcal{O}\left(\frac{L}{N^{k-2}}\right)
    %\end{equation*}
%\end{restatable}

%\begin{restatable}[Approximation Error]{thm}{ApproxErr}
%\label{approx_error}
    %If $u(t)$ is L-Lipschitz and twice differentiable and $\dot{u}(t)$ is M-Lipschitz, then the following holds for HiPPO LegS:
    %\begin{equation*}
    %\|\dot{u}(t) - \dot{u}_N(t)\|_2 \in \mathcal{O}\left(\sqrt{\frac{L^2 + LMt + M^2t}{N}}\right)
    %\end{equation*}
%\end{restatable}

%As a corollary of the above, we get that:

%\begin{restatable}[Approximation Error]{cor}{ApproxErrCor}
%\label{cor:ApproxErrCor}
    %Under the same assumptions and parametrization as in Theorem \ref{approx_error}, we have that:

     %\begin{equation*}
        % \left|u(t) - \widehat{u}_N(t)\right| \in \mathcal{O}\left(\frac{Lt}{N^{k-2}}\right)
      %\end{equation*}
    
%\end{restatable}

%\begin{restatable}[Approximation Error]{cor}{ApproxErrCor}
%\label{cor:ApproxErrCor}
    %Under the same assumption as in Theorem \ref{approx_error}, we have that for Hippo-LegS:
    %\begin{equation*}
       % \|u(t) - u_N(t)\|_2 
    %\in \mathcal{O}\left(t\sqrt{\frac{L^2 + LMt + t^2}{N}}\right)
    %\end{equation*}
%\end{restatable}

%As we expect, we have that the error decreases as N increases, i.e. as we consider more basis into the approximation and increases over time.\\
%For completeness, we will also report a global guarantee for the L2-error of $\dot{u}_N(s)$ and a fixed $t$. In particular, we have the following result:

%\begin{restatable}
    %[Global Approximation Error]{thm}{GlobalApproxErr}
    %If $u$ has k-th bounded derivatives with $k \geq 2$, then for the FouT parametrization it holds that:

    %\begin{equation*}
        %\|\dot{u} - \dot{u}_N\|_{2,\omega}^2 \in \mathcal{O}\left(\frac{L^2}{N^{2k-3}}{}\right)
    %\end{equation*}
    
%\end{restatable}



==> sections_submission_old/main_figure.tex <==
\begin{figure*}[t]
\centering
\subfigure[\small FouT and LegT on Van der Pol]{
    \includegraphics[width=0.31\textwidth]{figures/comparison_plot.pdf}
    \label{subfig:van_der_pol}
}
\hfill
\subfigure[\small Error dependence on $N, \alpha$]{
    \includegraphics[width=0.31\textwidth]{figures/filtered_vs_noise.pdf}
    \label{subfig:filtered_error}
}
\hfill
\subfigure[\small Error dependence on $N, \gamma$]{
    \includegraphics[width=0.31\textwidth]{figures/plot3_vs_noise.pdf}
    \label{subfig:whitenoise_error}
}

\vfill

\subfigure[\small Construction vs. trained LSSM]{
    \includegraphics[width=0.31\textwidth]{figures/bar_chart.pdf}
    \label{subfig:construction_vs_training}
}
\hfill
\subfigure[\small LegT error dependence on $t$]{
    \includegraphics[width=0.31\textwidth]{figures/error_vs_time_legt.pdf}
    \label{subfig:time_dependence}
}
\hfill
\subfigure[\small Filtered Noise \& White Signal]{
    \includegraphics[width=0.3\textwidth]{figures/example_signals.pdf}
    \label{subfig:example_signals}
}

\caption[Short Caption]{Empirical evaluation of our weight construction. \subfigref{subfig:van_der_pol} Van der Pol oscillator solution and errors of FouT and LegT weight construction. \subfigref{subfig:filtered_error} Error dependence on $N$ and low-pass filter strength $\alpha$ for the Filtered Noise dataset (mean across 1k functions and 1 std. plotted). \subfigref{subfig:whitenoise_error} Error dependence on $N$ and $\gamma$ for the White Signal dataset (mean across 1k functions and 1 std. plotted). \subfigref{subfig:construction_vs_training} Performance comparison of weight construction for LegT against different types of training: $(\mathrm{I})$ Initializing $\overline{\A},\overline{\B},\overline{\C},\overline{\D}$ at construction and training $\overline{\C},\overline{\D}$. $(\mathrm{II})$ Our weight construction. $(\mathrm{III})$ Initializing $\overline{\A},\overline{\B}$ at construction, random initialization and training of $\overline{\C},\overline{\D}$. $(\mathrm{IV})$ Initializing $\overline{\A},\overline{\B},\overline{\C},\overline{\D}$ at construction and training all of them (3 random seeds and error bars correspond to min and max). \subfigref{subfig:time_dependence} Error dependence of LegT on the context length $t$ on the White Signal Dataset (mean across 1k functions and 1 std. plotted). \subfigref{subfig:example_signals} Examples of the Filtered Noise ($\alpha = 0.05$) and White Signal ($\gamma = 2$) datasets}
\label{fig:label}
\end{figure*}



% \begin{figure*}[t]
% \centering
% \subfigure[Performance of FouT and LegT on Van der Pol oscillator]{
%     \includegraphics[width=0.33\textwidth]{figures/comparison_plot.pdf}
%     \label{subfig:van_der_pol}
% }
% \hfill
% \subfigure[Error dependence on $N$ and low-pass filter strength]{
%     \includegraphics[width=0.33\textwidth]{figures/filtered_vs_noise.pdf}
%     \label{subfig:filtered_error}
% }
% \hfill
% \subfigure[Error dependence on $N$ and signal frequency]{
%     \includegraphics[width=0.33\textwidth]{figures/filtered_vs_noise.pdf}
%     \label{subfig:whitenoise_error}
% }
% \hfill
% \subfigure[Weight construction vs. trained LSSM]{
%     \includegraphics[width=0.33\textwidth]{figures/bar_chart.pdf}
%     \label{subfig:diffusion_runtime}
% }
% \hfill
% \subfigure[Error dependence on context length LegT]{
%     \includegraphics[width=0.33\textwidth]{figures/error_vs_time_legt.pdf}
%     \label{subfig:strings_stat}
% }
% \hfill
% \subfigure[Example band limited and low passed white noise examples]{
%     \includegraphics[width=0.33\textwidth]{figures/filtered_vs_noise.pdf}
%     \label{subfig:example_signals}
% }
% \caption[Short Caption]{Empirical evaluation of our weight construction. (\subfigref{subfig:van_der_pol}) Van der Pol oscillator solution and errors of FouT and LegT weight construction. (\subfigref{subfig:filtered_error}) Error dependence on $N$ and low-pass filter strength. (\subfigref{subfig:whitenoise_error}) Error dependence on $N$ and signal frequency. (\subfigref{subfig:diffusion_runtime}) Weight construction vs. trained LSSM. (\subfigref{subfig:strings_stat}) Error dependence on context length LegT. (\subfigref{subfig:example_signals}) Example band limited and low passed white noise examples.}
% \label{fig:label}
% \end{figure*}


% % \begin{figure*}[t]
% % \centering
% % \subcaptionbox[Short Subcaption]{
% %     Performance of FouT and LegT on Van der Pol oscillator
% %     \label{subfig:van_der_pol}}
% % [
% %     0.33\textwidth % width of caption
% % ]
% % {%
% %     \includegraphics[width=0.33\textwidth]{figures/comparison_plot.pdf}%
% % }%
% % \hfill % seperation
% % \subcaptionbox[Short Subcaption]{%
% %     Error dependence on $N$ and low-pass filter strength
% %     \label{subfig:filtered_error}%
% % }
% % [%
% %     0.33\textwidth % width of caption
% % ]%
% % {%
% %     \includegraphics[width=0.33\textwidth]{figures/filtered_vs_noise.pdf}%
% % }% 
% % \hfill
% % \subcaptionbox[Short Subcaption]{%
% %     Error dependence on $N$ and signal frequency
% %     \label{subfig:whitenoise_error}%
% % }
% % [%
% %     0.33\textwidth % width of caption
% % ]%
% % {%
% %     \includegraphics[width=0.33\textwidth]{figures/filtered_vs_noise.pdf}%
% % }% 
% % \hfill
% % \subcaptionbox[Short Subcaption]{%
% %    Weight construction vs. trained LSSM
% % \label{subfig:diffusion_runtime}%
% % }
% % [%
% %     0.33\textwidth % width of caption
% % ]%
% % {%
% %     \includegraphics[width=0.33\textwidth]{figures/bar_chart.pdf}%
% % }%
% % \hfill
% % \subcaptionbox[Short Subcaption]{%
% %     Error dependence on context length LegT%
% %     \label{subfig:strings_stat}%
% % }
% % [%
% %     0.33\textwidth % width of caption
% % ]%
% % {%
% %     \includegraphics[width=0.33\textwidth]{figures/error_vs_time_legt.pdf}%
% % }%
% % \hfill
% % \subcaptionbox[Short Subcaption]{%
% %     Example band limited and low passed white noise examples
% %     \label{subfig:example_signals}%
% % }
% % [%
% %     0.33\textwidth % width of caption
% % ]%
% % {%
% %     \includegraphics[width=0.33\textwidth]{figures/filtered_vs_noise.pdf}%
% % }%
% % \caption[Short Caption]{\looseness -1 Empirical evaluation of our weight construction.\ref{subfig:van_der_pol} Van der Pol oscillator solution and errors of FouT and LegT weight construction. \ref{subfig:filtered_error} Error de}
% % \label{fig:label}
% % \end{figure*}

==> sections_submission_old/old_proofs.tex <==
\ApproxErr*

\begin{proof}
Assuming that we can exchange sum and derivative, we have
\begin{align}
    \|\dot{u}(t) - \dot{u}_N(t)\|_2^2 &= \sum_{n \geq N} |\dot{x}_n(t)|^2
\end{align}

\color{red} I found out this is probably a mistake as in our case, the way we derived $\dot{u}(t)$, the $\dot{x}_n(t)$ are not the coefficients of the Fourier expansion wrt Lagrange basis but for some other (probably not orthogonal basis) and hence they do not respect Parseval's identity. I am now trying to find a way to fix this by changing the construction and deriving first an expression of $\dot{u}(s)$ from Equation 2 (i.e. by first taking derivative wrt to s and then evaluate at t) wrt Lagrange basis so that we can use this for the analysis. I was actually thinking for this to use classic Fourier basis instead (sines and cosines) as the analysis is much easier (derivatives of Legendre polynomials are a mess). I think we can still use our construction for experiments (although we won't have a guarantee for that) and then use this Fourier basis for theoretical analysis (and maybe also compare in experiments). \color{black}

by the Parseval identity, where here we indicate $\dot{u}_N(t)$ as the output of our model and $\dot{u}(t)$ the true derivative of the input.\\
If we use the HiPPo-LegS parametrization, we get that (see \citep{NEURIPS2020_102f0bb6} or \citep{gu2022train}  for further details):
\begin{equation}
    x_n(t) = \frac{\sqrt{2n+1}}{t}\int_0^t u(s) P_n\left(\frac{2s}{t} -1\right)\mathrm{d}s 
\end{equation}
Then, we have:
\begin{align*}
    \dot{x}_n(t) &= \frac{\mathrm{d}}{\mathrm{d}t} \left( \frac{\sqrt{2n+1}}{t}\int_0^t u(s) P_n\left(\frac{2s}{t} -1\right)\mathrm{d}s \right)\\
    &=\frac{\mathrm{d}}{\mathrm{d}t} \left( \frac{\sqrt{2n+1}}{2}\int_{-1}^1 u\left(\frac{1 + y}{2}t\right)P_n(y)\mathrm{d}y \right) \ \ \ \ \ \text{by the change of variables $y = \frac{2s}{t}-1$}\\
    &=\frac{\mathrm{d}}{\mathrm{d}t} \left(- \frac{t}{4\sqrt{2n+1}}\int_{-1}^1 \dot{u}\left(\frac{1 + y}{2}t\right)\Big(P_{n+1}(y) - P_{n-1}(y)\Big)\mathrm{d}y \right)
\end{align*}

where in the last step we integrated by parts using the fact that $P_n(y)=\frac{1}{2n+1}\frac{\mathrm{d}}{\mathrm{d}y}(P_{n+1}(y)-P_{n-1}(y))$ and noticed that the boundary terms cancel since $P_{n+1}(y)=P_{n-1}(y)$ for $y=\pm 1$. Then, by applying the product rule, we have that:

\begin{multline}
    \dot{x}_n(t) = - \frac{1}{4\sqrt{2n+1}}\int_{-1}^1 \dot{u}\left(\frac{1 + y}{2}t\right)\Big(P_{n+1}(y) - P_{n-1}(y)\Big)\mathrm{d}y\\
    - \frac{t}{4\sqrt{2n+1}}\int_{-1}^1 \frac{1 + y}{2}\ddot{u}\left(\frac{1 + y}{2}t\right)\Big(P_{n+1}(y) - P_{n-1}(y)\Big)\mathrm{d}y 
\end{multline}

Hence, we get the following expression for the terms of the infinite series we want to bound:
\begin{align*}
    |\dot{x}_n(t)|^2 =&\: \frac{1}{16}\frac{1}{2n+1}\left(\int_{-1}^1 \dot{u}\left(\frac{1 + y}{2}t\right)\Big(P_{n+1}(y) - P_{n-1}(y)\Big)\mathrm{d}y \right)^2\\
    &+ \frac{1}{16}\frac{t^2}{2n+1}\left(\int_{-1}^1 \frac{1+y}{2}\ddot{u}\left(\frac{1+y}{2}t\right)\Big(P_{n+1}(y) - P_{n-1}(y)\Big)\mathrm{d}y\right)^2\\
    &+\frac{1}{8}\frac{t}{2n+1}\left(\int_{-1}^1 \dot{u}\left(\frac{1 + y}{2}t\right)\Big(P_{n+1}(y) - P_{n-1}(y)\Big)\mathrm{d}y\right)\\
    &\:\:\:\:\:\left(\int_{-1}^1 \frac{1+y}{2}\ddot{u}\left(\frac{1+y}{2}t\right) \Big(P_{n+1}(y) - P_{n-1}(y)\Big)\mathrm{d}y\right)
\end{align*}
We now bound all the three terms individually.
\begin{align*}
    &\:\:\:\:\:\:\frac{1}{16}\frac{1}{2n+1}\Bigg(\int_{-1}^1 \dot{u}\left(\frac{1 + y}{2}t\right)\Big(P_{n+1}(y) - P_{n-1}(y)\Big)\mathrm{d}y \Bigg)^2\\
    &\labelrel\leq{step:term1_1} \frac{L^2}{16(2n+1)}\left(\int_{-1}^1 P_{n+1}(y) - P_{n-1}(y) \mathrm{d}y\right)^2 \\
    &\labelrel\leq{step:term1_2} \frac{L^2}{8(2n+1)} \int_{-1}^1 \Big(P_{n+1}(y) - P_{n-1}(y)\Big)^2 \mathrm{d}y \\
    &\labelrel={step:term1_3} \frac{L^2}{8(2n+1)} \left(\int_{-1}^1 P_{n+1}(y)^2\mathrm{d}y +\int_{-1}^1 P_{n-1}(y)^2\mathrm{d}y\right) \\
    &=\frac{L^2}{8(2n+1)}\left( \frac{2}{2n+2} + \frac{2}{2n + 1}\right) \\
    &\in \mathcal{O}\left(\frac{L^2}{n^2}\right)
\end{align*}
where in \eqref{step:term1_1} we use the fact that $u$ is $L$-Lipschitz and hence $\dot{u}(t)\leq L$, in \eqref{step:term1_2} we use Cauchy-Schwarz and in \eqref{step:term1_3} we use the fact that $P_{n+1}(y)$ and $P_{n-1}(y)$ are orthogonal and hence their inner product vanishes. \\
Then, for the second term we have:

\begin{align*}
    &\:\:\:\:\:\:\frac{1}{16}\frac{t^2}{2n+1}\Bigg(\int_{-1}^1 \frac{1+y}{2}\ddot{u}\Bigg(\frac{1+y}{2}t\Bigg)\Big(P_{n+1}(y) - P_{n-1}(y)\Big)\mathrm{d}y\Bigg)^2\\
    &\leq \frac{t^2M^2}{16(2n+1)}
    \left(\int_{-1}^1 P_{n+1}(y) - P_{n-1}(y) \mathrm{d}y \right)^2 \\
    &\in \mathcal{O}\left(\frac{t^2M^2}{n^2}\right)
\end{align*}

where we used the fact that $\dot{u}$ is M-Lipschitz and that $\frac{1+y}{2} \leq 1$ for $y \in [-1, 1]$.\\
Finally, for the third term we have:

\begin{align*}
    &\:\:\:\:\:\:\frac{1}{8}\frac{1}{2n+1}\left(\int_{-1}^1 \dot{u}\left(\frac{1 + y}{2}t\right)\left(P_{n+1}(y) - P_{n-1}(y)\right)\mathrm{d}y\right)\\  
    &\:\:\:\:\:\:\cdot\left(\int_{-1}^1 \frac{1+y}{2}\ddot{u}\left(\frac{1+y}{2}t\right) \left(P_{n+1}(y) - P_{n-1}(y)\right)\mathrm{d}y\right)\\
    &\leq \frac{LMt}{8(2n+1)}\left(\int_{-1}^1 P_{n+1}(y) - P_{n-1}(y) \mathrm{d}y \right)^2\\
    &\in \mathcal{O}\left(\frac{LMt}{n^2}\right)
\end{align*}

where again we used the Lipschitz conditions and the fact that $\frac{1+y}{2} \leq 1$ for $y \in [-1, 1]$. \\
Therefore, by summing all the terms, we conclude that:
\begin{equation*}
    \|\dot{u}(t) - \dot{u}_N(t)\|_2^2 \in \mathcal{O}\left(\frac{L^2 + LMt + M^2t}{N}\right)
\end{equation*}

and as a consequence:

\begin{equation*}
    \|\dot{u}(t) - \dot{u}_N(t)\|_2 \in \mathcal{O}\left(\sqrt{\frac{L^2 + LMt + M^2t}{N}}\right)
\end{equation*}
\end{proof}

\ApproxErrCor*

\begin{proof}
\begin{align*}
    \|u(t) - u_N(t)\|_2 &= \bigg|\int_{0}^t\dot{u}(s) - \dot{u}_N(s)\mathrm{d}s\bigg|\\ &\leq \int_{0}^t\big|\dot{u}(s) - \dot{u}_N(s)\big| \mathrm{d}s\\
    &\leq \int_{0}^t \mathcal{O}(1) \sqrt{\frac{L^2 + LMs + M^2s^2}{N}}  \mathrm{d}s\\
    &\labelrel\leq{step:cor} \int_{0}^t \mathcal{O}(1) \sqrt{\frac{L^2 + LMt + M^2t^2}{N}} \mathrm{d}s\\
    &\in \mathcal{O}\left(t\sqrt{\frac{L^2 + LMt + t^2}{N}}\right)
\end{align*}
where in ~\eqref{step:cor} we used that $\sqrt{(L^2 + LMs + M^2s^2)/N}$ is monotonically increasing in $[0, t]$.
\end{proof}

==> sections_submission_old/old_proofs_old.tex <==
\ApproxErr*

\begin{proof}
Assuming that we can exchange sum and derivative, we have
\begin{align}
    \|\dot{u}(t) - \dot{u}_N(t)\|_2^2 &= \sum_{n \geq N} |\dot{x}_n(t)|^2
\end{align}

\color{red} I found out this is probably a mistake as in our case, the way we derived $\dot{u}(t)$, the $\dot{x}_n(t)$ are not the coefficients of the Fourier expansion wrt Lagrange basis but for some other (probably not orthogonal basis) and hence they do not respect Parseval's identity. I am now trying to find a way to fix this by changing the construction and deriving first an expression of $\dot{u}(s)$ from Equation 2 (i.e. by first taking derivative wrt to s and then evaluate at t) wrt Lagrange basis so that we can use this for the analysis. I was actually thinking for this to use classic Fourier basis instead (sines and cosines) as the analysis is much easier (derivatives of Legendre polynomials are a mess). I think we can still use our construction for experiments (although we won't have a guarantee for that) and then use this Fourier basis for theoretical analysis (and maybe also compare in experiments). \color{black}

by the Parseval identity, where here we indicate $\dot{u}_N(t)$ as the output of our model and $\dot{u}(t)$ the true derivative of the input.\\
If we use the HiPPo-LegS parametrization, we get that (see \citep{NEURIPS2020_102f0bb6} or \citep{gu2022train}  for further details):
\begin{equation}
    x_n(t) = \frac{\sqrt{2n+1}}{t}\int_0^t u(s) P_n\left(\frac{2s}{t} -1\right)\mathrm{d}s 
\end{equation}
Then, we have:
\begin{align*}
    \dot{x}_n(t) &= \frac{\mathrm{d}}{\mathrm{d}t} \left( \frac{\sqrt{2n+1}}{t}\int_0^t u(s) P_n\left(\frac{2s}{t} -1\right)\mathrm{d}s \right)\\
    &=\frac{\mathrm{d}}{\mathrm{d}t} \left( \frac{\sqrt{2n+1}}{2}\int_{-1}^1 u\left(\frac{1 + y}{2}t\right)P_n(y)\mathrm{d}y \right) \ \ \ \ \ \text{by the change of variables $y = \frac{2s}{t}-1$}\\
    &=\frac{\mathrm{d}}{\mathrm{d}t} \left(- \frac{t}{4\sqrt{2n+1}}\int_{-1}^1 \dot{u}\left(\frac{1 + y}{2}t\right)\Big(P_{n+1}(y) - P_{n-1}(y)\Big)\mathrm{d}y \right)
\end{align*}

where in the last step we integrated by parts using the fact that $P_n(y)=\frac{1}{2n+1}\frac{\mathrm{d}}{\mathrm{d}y}(P_{n+1}(y)-P_{n-1}(y))$ and noticed that the boundary terms cancel since $P_{n+1}(y)=P_{n-1}(y)$ for $y=\pm 1$. Then, by applying the product rule, we have that:

\begin{multline}
    \dot{x}_n(t) = - \frac{1}{4\sqrt{2n+1}}\int_{-1}^1 \dot{u}\left(\frac{1 + y}{2}t\right)\Big(P_{n+1}(y) - P_{n-1}(y)\Big)\mathrm{d}y\\
    - \frac{t}{4\sqrt{2n+1}}\int_{-1}^1 \frac{1 + y}{2}\ddot{u}\left(\frac{1 + y}{2}t\right)\Big(P_{n+1}(y) - P_{n-1}(y)\Big)\mathrm{d}y 
\end{multline}

Hence, we get the following expression for the terms of the infinite series we want to bound:
\begin{align*}
    |\dot{x}_n(t)|^2 =&\: \frac{1}{16}\frac{1}{2n+1}\left(\int_{-1}^1 \dot{u}\left(\frac{1 + y}{2}t\right)\Big(P_{n+1}(y) - P_{n-1}(y)\Big)\mathrm{d}y \right)^2\\
    &+ \frac{1}{16}\frac{t^2}{2n+1}\left(\int_{-1}^1 \frac{1+y}{2}\ddot{u}\left(\frac{1+y}{2}t\right)\Big(P_{n+1}(y) - P_{n-1}(y)\Big)\mathrm{d}y\right)^2\\
    &+\frac{1}{8}\frac{t}{2n+1}\left(\int_{-1}^1 \dot{u}\left(\frac{1 + y}{2}t\right)\Big(P_{n+1}(y) - P_{n-1}(y)\Big)\mathrm{d}y\right)\\
    &\:\:\:\:\:\left(\int_{-1}^1 \frac{1+y}{2}\ddot{u}\left(\frac{1+y}{2}t\right) \Big(P_{n+1}(y) - P_{n-1}(y)\Big)\mathrm{d}y\right)
\end{align*}
We now bound all the three terms individually.
\begin{align*}
    &\:\:\:\:\:\:\frac{1}{16}\frac{1}{2n+1}\Bigg(\int_{-1}^1 \dot{u}\left(\frac{1 + y}{2}t\right)\Big(P_{n+1}(y) - P_{n-1}(y)\Big)\mathrm{d}y \Bigg)^2\\
    &\labelrel\leq{step:term1_1} \frac{L^2}{16(2n+1)}\left(\int_{-1}^1 P_{n+1}(y) - P_{n-1}(y) \mathrm{d}y\right)^2 \\
    &\labelrel\leq{step:term1_2} \frac{L^2}{8(2n+1)} \int_{-1}^1 \Big(P_{n+1}(y) - P_{n-1}(y)\Big)^2 \mathrm{d}y \\
    &\labelrel={step:term1_3} \frac{L^2}{8(2n+1)} \left(\int_{-1}^1 P_{n+1}(y)^2\mathrm{d}y +\int_{-1}^1 P_{n-1}(y)^2\mathrm{d}y\right) \\
    &=\frac{L^2}{8(2n+1)}\left( \frac{2}{2n+2} + \frac{2}{2n + 1}\right) \\
    &\in \mathcal{O}\left(\frac{L^2}{n^2}\right)
\end{align*}
where in \eqref{step:term1_1} we use the fact that $u$ is $L$-Lipschitz and hence $\dot{u}(t)\leq L$, in \eqref{step:term1_2} we use Cauchy-Schwarz and in \eqref{step:term1_3} we use the fact that $P_{n+1}(y)$ and $P_{n-1}(y)$ are orthogonal and hence their inner product vanishes. \\
Then, for the second term we have:

\begin{align*}
    &\:\:\:\:\:\:\frac{1}{16}\frac{t^2}{2n+1}\Bigg(\int_{-1}^1 \frac{1+y}{2}\ddot{u}\Bigg(\frac{1+y}{2}t\Bigg)\Big(P_{n+1}(y) - P_{n-1}(y)\Big)\mathrm{d}y\Bigg)^2\\
    &\leq \frac{t^2M^2}{16(2n+1)}
    \left(\int_{-1}^1 P_{n+1}(y) - P_{n-1}(y) \mathrm{d}y \right)^2 \\
    &\in \mathcal{O}\left(\frac{t^2M^2}{n^2}\right)
\end{align*}

where we used the fact that $\dot{u}$ is M-Lipschitz and that $\frac{1+y}{2} \leq 1$ for $y \in [-1, 1]$.\\
Finally, for the third term we have:

\begin{align*}
    &\:\:\:\:\:\:\frac{1}{8}\frac{1}{2n+1}\left(\int_{-1}^1 \dot{u}\left(\frac{1 + y}{2}t\right)\left(P_{n+1}(y) - P_{n-1}(y)\right)\mathrm{d}y\right)\\  
    &\:\:\:\:\:\:\cdot\left(\int_{-1}^1 \frac{1+y}{2}\ddot{u}\left(\frac{1+y}{2}t\right) \left(P_{n+1}(y) - P_{n-1}(y)\right)\mathrm{d}y\right)\\
    &\leq \frac{LMt}{8(2n+1)}\left(\int_{-1}^1 P_{n+1}(y) - P_{n-1}(y) \mathrm{d}y \right)^2\\
    &\in \mathcal{O}\left(\frac{LMt}{n^2}\right)
\end{align*}

where again we used the Lipschitz conditions and the fact that $\frac{1+y}{2} \leq 1$ for $y \in [-1, 1]$. \\
Therefore, by summing all the terms, we conclude that:
\begin{equation*}
    \|\dot{u}(t) - \dot{u}_N(t)\|_2^2 \in \mathcal{O}\left(\frac{L^2 + LMt + M^2t}{N}\right)
\end{equation*}

and as a consequence:

\begin{equation*}
    \|\dot{u}(t) - \dot{u}_N(t)\|_2 \in \mathcal{O}\left(\sqrt{\frac{L^2 + LMt + M^2t}{N}}\right)
\end{equation*}
\end{proof}

\ApproxErrCor*

\begin{proof}
\begin{align*}
    \|u(t) - u_N(t)\|_2 &= \bigg|\int_{0}^t\dot{u}(s) - \dot{u}_N(s)\mathrm{d}s\bigg|\\ &\leq \int_{0}^t\big|\dot{u}(s) - \dot{u}_N(s)\big| \mathrm{d}s\\
    &\leq \int_{0}^t \mathcal{O}(1) \sqrt{\frac{L^2 + LMs + M^2s^2}{N}}  \mathrm{d}s\\
    &\labelrel\leq{step:cor} \int_{0}^t \mathcal{O}(1) \sqrt{\frac{L^2 + LMt + M^2t^2}{N}} \mathrm{d}s\\
    &\in \mathcal{O}\left(t\sqrt{\frac{L^2 + LMt + t^2}{N}}\right)
\end{align*}
where in ~\eqref{step:cor} we used that $\sqrt{(L^2 + LMs + M^2s^2)/N}$ is monotonically increasing in $[0, t]$.
\end{proof}

==> sections_submission_old/problem_formulation.tex <==
\section{SSMs and HiPPO Theory}
% \color{red} TODO: introduce discretized systems as well \color{black} 
LSSMs map an input signal $u(t) \in \mathbb{R}$ to an output signal $y(t) \in \mathbb{R}$ via a hidden state $x(t) \in \mathbb{R}^N$ and take the following form:
\begin{equation}
    \begin{cases}
        \dot{x}(t) = \A x(t)+\B u(t) \\
        y(t) = \C x(t)+\D u(t)
    \end{cases}
\end{equation}
One key property of these models is their ability to memorize past information, $u(s)$ for $s\leq t$, 
in their hidden state $x(t)$. This capability was established in the HiPPO framework \cite{NEURIPS2020_102f0bb6,gu2022train}. 
More formally, HiPPO theory considers a Hilbert space spanned by the orthogonal basis functions $\{ p_n(t,s)\}_{n \geq 0}$, equipped with a measure $\omega(t,s)$ and an inner product $\langle f, g \rangle_\omega = \int_{-\infty}^t f(s)g(s) \omega(t,s) \mathrm{d}s$. The theory shows a way to construct $\A$ and $\B$ such that the hidden state $x_n(t)$ represents the projection of the input signal $u_{\leq t}$ onto the basis $p_n(t,s)$ i.e. $x_n(t) = \langle u_{\leq t}, p_n \rangle_\omega$.
 %We are going to review two of the methods proposed by HiPPO theory, their choice of basis and their respective constructions of $\A$ and $\B$ later in this section. 
One of the fundamental results in HiPPO theory is that in the limit of an infinite hidden state size $N \rightarrow \infty$ and for an appropriate choice of $\A$ and $\B$, it is possible to reconstruct the input signal up to time $t$ from the hidden state $x(t)$:
\begin{equation}
\label{reconstruction}
    u(s) = \sum_{n=0}^{\infty} x_n(t) p_n(t,s) \ \ \forall s\leq t
\end{equation}
In this work, we consider three specific HiPPO parameterizations of $\A$ and $\B$: LegT and LegS based on Legendre polynomials, and FouT which is based on Fourier basis. The explicit constructions for $\A$ and $\B$ are given in Appendix \ref{parametrizations}.
\section{Solving Dynamical Systems with SSMs}
To investigate the autoregressive ICL capabilities of LSSMs we build on HiPPO theory and establish a way to predict the future time step $u(t+\Delta t)$ of a dynamical system. To do so, we need to approximate the following integral, having access to $u(t)$:
%To investigate the autoregressive ICL capabilities of LSSMs we consider a dynamical system of the form $\dot{u}(t) = \Phi(u, t)$. The task of the model is to predict the next state $u(t + \Delta t)$, given the history $u_{\leq t}$. To this end, we extend the HiPPO framework to analyze the ability of continuous LSSMs to predict the next state of a first order dynamical system. To predict a future time-step $u(t+\Delta t)$, we need to approximate the following integral, having access to $u(t)$:
\begin{equation}\label{eq: disc}
    u(t+\Delta t) = u(t) +\int_{t}^{t+\Delta t}\dot{u}(s) \mathrm{d}s
\end{equation}
To this end, \textbf{(1)} we approximate $\dot{u}(t)$ in the continuous time setting by constructing a specific parameterization for $\C$ and $\D$ for a general basis $\{p_n\}_{n \geq 0}$ resulting in a model satisfying $\dot{u}(t) \approx y(t)=\C x(t)+\D u(t)$. Subsequently, \textbf{(2)} we show how to approximate the integral via discretization. Finally, \textbf{(3)}, we provide an asymptotic bound on the error incurred by approximating $\dot{u}(t)$. 
\par
% HiPPO theory provides many different constructions for the matrices $\A$ and $\B$, but here we will focus on three of them in particular, namely HiPPO-LegT, HiPPO-LegS and HiPPO-FouT. The first two of them rely on projections on the space of Legendre polynomials, the first leading to a LTI system whereas the second leads to a time-varying system. The latter instead leverages projections on the space of Fourier basis, made of classical sine and cosine basis functions. 
% As mentioned above, the main goal of HiPPo theory is to construct matrices $A$ and $B$ to show that $x(t)$ is able to retain all the information about the input signal up until that point and only based on this information we can approximately reconstruct the signal until time $t$. However, this approach only focused on $A$, $B$ and $x(t)$ but never really considered $C$, $D$ and $y(t)$. In our work, we aim to leverage these to predict the value of the input at the next time step.
%More precisely, our goal will be, for each of the three aforementioned constructions of HiPPO Theory, to find a parametrization of $\C$ and $\D$ such that the output $y(t)$ corresponds to $\dot{u}(t)$ (in the limit of $N \rightarrow \infty)$. Note that once we have this equivalence, we can discretize the equation $\dot{u}(t) \approx y(t)=\C x(t)+\D u(t)$ in order to get an approximation of the next input.
%Note that \citep{gu2022train} and \citep{NEURIPS2020_102f0bb6} analyze the HiPPO theory in the continuous setting of SSMs as in this case it is more natural to construct Hilbert spaces with inner products and their parametrizations for $\A$ and $\B$. Only after they derived these parametrizations they discretize the system so that we can leverage this approach in practice as well. We will follow a similar approach: we will first derive the parametrization for $\C$ and $\D$ in the continuous setting as this has analytical and theoretical advantages and then we will derive their discretized versions that we will use in our experiments.
\textbf{(1)} We focus on LegT and FouT, and provide LegS in Appendix \ref{app:legs}.
By evaluating Equation \ref{reconstruction} at time $t$, we get: $u(t) = \sum_{n=0}^{\infty} x_n(t) p_n(t,t)$. Under some technical assumptions we can exchange the series with the derivative\footnote{If $f(x)=\sum_{n=0}^\infty f_n(x)$, then if $\sum_{n=0}^\infty \dot{f}_n(x)$ converges absolutely we have that $\dot{f}(x)=\sum_{n=0}^\infty \dot{f}_n(x)$. We will assume this assumption holds throughout the rest of the paper and test it empirically.}. Noting that $p_n(t,t)$ is a constant w.r.t $t$, we get $\dot{u}(t) = \sum_{n=0}^{\infty} \dot{x}_n(t) p_n(t,t)$. Through this, we establish a weight construction in Prop. \ref{prop:construction_legt_fout}, through which the gradient of the input signal can be approximated.
%Starting from Equation \ref{u_t_dec}, we will construct the matrices $C$ and $D$ for the three methods. We will separate the two cases and we will first review the differences in these two methods, e.g. which basis and measure they assume and their different parametrizations of $\A$ and $\B$.
% As mentioned above, HiPPO-LegT uses Legendre polynomials as their basis functions. In particular, we have that $\omega(t,s)= \frac{1}{\theta}\mathbb{1}_{[t-\theta, t]}(s)$ and $p_n(t,s)=\sqrt{2n+1}P_n(2\frac{s-t}{\theta}+1)$ where $P_n$ is the nth Legendre polynomial. This leads to the following choice for $\A$ and $\B$:
% \begin{align}
%     \A_{nk} = \frac{1}{\theta} \begin{cases}
%         (-1)^{n-k}(2n+1) \ \ \ \text{if $n \geq k$}\\
%         (2n+1) \ \ \ \text{if $n < k$}
%     \end{cases} 
%     \ \ \ \ \ \ 
%     \B_n=\frac{1}{\theta}(2n+1)(-1)^n
% \end{align}
% Then, the following holds for the construction of $\C$ and $\D$:
\begin{restatable}[Construction of $\C$ and $\D$ for LegT and FouT]{prop}{ConstrLegTFouT}
    \label{prop:construction_legt_fout}
    If we choose $\C_j = \sum_{k = 0}^N\A_{kj}p_k(t, t)$ and $
    \D = \sum_{k = 0}^N \B_k p_k(t, t)$ and $\A$, $\B$ and $p_k(t,t)$ as in HiPPO LegT or FouT, then the output $y(t)$ is an approximation of $\dot{u}(t)$ based on $N$ basis functions.
\end{restatable}
%\vspace{3mm}
%\subsection{HiPPo-LegS}
%  HiPPO-LegS also uses Legendre polynomials as their basis functions. However, here we have that $\omega(t,s)= \frac{1}{t}\mathbb{1}_{[0, t]}(s)$ and $p_n(t,s)=\sqrt{2n+1}P_n(\frac{2s}{t}-1)$ where $P_n$ again is the nth Legendre polynomial. Note that whereas the measure of LegT is translation invariant, the measure of LegS is not. This causes the system to become Time-Varying and in particular this leads to having $\dot{x}(t)=-\frac{1}{t}Ax(t)+\frac{1}{t}Bu(t)$ with the following choice for $\A$ and $\B$:
% \begin{align}
%     \A_{nk} =  \begin{cases}
%         \sqrt{2n+1}\sqrt{2k+1} \ \ \ \text{if $n > k$}\\
%         (n+1) \ \ \ \text{if $n = k$}\\
%         0 \ \ \ \text{o.w.}
%     \end{cases} 
%     \ \ \ \ \ \ 
%     \B_n=\sqrt{2n+1}
% \end{align}
%Then, the following result holds for $\C$ and $\D$
% \begin{restatable}[LegS construction]{prop}{LegS}
%     \label{prop:LegS}
%     If we choose $\C_j = \sum_{k = 0}^N\frac{1}{t}\A_{kj}p_k(t, t)$ and $
%     \D = \sum_{k = 0}^N \frac{1}{t}\B_k p_k(t, t)$ and $\A$, $\B$ and $p_k(t,t)$ as in HiPPO LegS, then the output $y(t)$ is an approximation of $\dot{u}(t)$ based on $N$ basis functions.
% \end{restatable}
% \vspace{3mm}
%\subsection{HiPPO-FouT}
%We now propose a different way to derive $\dot{u}(t)$ from Equation \ref{reconstruction}, which we will base our theoretical analysis on. In particular, instead of first evaluating $u(s)$ at $t$ and then taking the derivative, we will first derive $u(s)$ and only then evaluate the function at $t$. For the construction of $\C$ and $\D$, we will use the classic Fourier basis of sines and cosines to make the analysis easier, although the derivation of $\dot{u}(t)$ remains valid for any choice of basis functions. In particular, we have the following:

%\begin{equation}
    %\dot{u}(s) = \sum_{n=0}^{\infty} x_n(t) \frac{\partial}{\partial s}p_n(t,s) \ \ \forall s < t
%\end{equation}

%Note that by assuming continuity of $\dot{u}$ and $p_n$ wrt $s$, we can take the limit from the left as $s$ goes to $t$, giving us:

%\begin{equation}
    %\dot{u}(t) = \sum_{n=0}^{\infty} x_n(t) \frac{\partial}{\partial s}p_n(t,s) \Big |_{s=t} 
%\end{equation}

% HiPPo-FouT, differently from LegT and LegS uses the classical Fourier basis and in particular it assumes $\{p_n\}_{n \geq 0}(t,s) = \sqrt{2} \Big [1 \ \cos(2\pi [1-(t-s)]) \ \sin(2\pi [1-(t-s)] \ \cos(4\pi [1-(t-s)] \ \sin(4\pi [1-(t-s)]) \ \dots \Big]$ and $\omega(t,s)= \mathbb{1}_{[t-1, t]}(s)$. This leads to the following choice of $\A$ and $\B$:

% \begin{align}
%     A_{nk} = 
%     \begin{cases}
%         -2 \ \ \ \text{if $n=k=0$}\\
%         -2\sqrt{2} \ \ \ \text{if $n=0$ and $k$ odd or $k=0$ and $n$ odd}\\
%         -4 \ \ \ \text{if $n$ odd and $k$ odd}\\
%         2\pi n \ \ \ \text{if $n-k=1$ and $k$ odd}\\
%         -2\pi k \ \ \ \text{if $k-n=1$ and $n$ odd}\\
%         0 \ \ \ \text{o.w.}
%     \end{cases}
%     \ \ \ \ 
%     B_n= 
%     \begin{cases}
%         2 \ \ \ \text{if $n=0$}\\
%         2 \sqrt{2} \ \ \ \text{if $n$ odd}\\
%         0 \ \ \ \text{o.w.}
%     \end{cases}
% \end{align}

%We now have the following result for construction of $\C$ and $\D$ for FouT:

% \begin{restatable}[FouT construction]{prop}{FouT}
% \label{fout}
% If we choose $\C_j = \sum_{k = 0}^N\A_{kj}p_k(t, t)$ and $
%     \D = \sum_{k = 0}^N \B_k p_k(t, t)$ and $\A$, $\B$ and $p_k(t,t)$ as in HiPPO FouT, then the output $y(t)$ is an approximation of $\dot{u}(t)$ based on $N$ basis functions.
% \end{restatable}

% \vspace{3mm}
% \subsection{Discretization}
%\color{red} Introduce discretization for general linear systems \color{black}
% Note that to predict the next time-step $u(t+\Delta t)$, we need to approximate the following integral, having access to $u(t)$:
% \begin{equation}
%     u(t+\Delta t) = u(t) +\int_{t}^{t+\Delta t}\dot{u}(s) ds
% \end{equation}
%\color{red} Introduce discretization for general linear systems \color{black}\\
\textbf{(2)} Since we cannot solve the integral in Equation \ref{eq: disc} in closed form, we approximate it using the bilinear method which was found to work well in practice \cite{NEURIPS2020_102f0bb6}. %Note that we could use any other discretization methods (e.g. Forward/Backward Euler or Generalized Bilinear Transformation), but here we stick with the choice of the Bilinear method which is the most common one and exhibits nice stability properties. 
This leads to the following approximation, the derivation of which can be found in Appendix \ref{app:discretization}:
\begin{align} \label{CD}
    \widehat{u}_{k+1} 
    &\approx \left( 1 - \frac{\D \Delta t}{2}\right)^{-1} \left[ \left( 1 + \frac{\D \Delta t}{2}\right)u_k + \Delta t \C x_{k+1} \right]
    = \overline{\C} x_{k+1} + \overline{\D} u_k
\end{align}
where $\C$ and $\D$ are the parametrizations of HiPPO LegT or FouT from Proposition \ref{prop:construction_legt_fout}. In the discrete-time system, we have $x_{k+1} = \overline{\A} x_{k}+\overline{\B} u_k$, where \smash{$\overline{\A} = (I-\frac{\Delta t}{2}\A)^{-1}(I+\frac{\Delta t}{2}\A)$} and \smash{$\overline{\B} = \Delta t (I-\frac{\Delta t}{2}\A)^{-1}\B$} are the discretized versions of $\A$ and $\B$ \citep{NEURIPS2020_102f0bb6}, resulting in:
\begin{equation}
\label{discretized_sys}
    \begin{cases}
    x_{k+1} = \overline{\A} x_{k}+\overline{\B} u_k \\
    \widehat{u}_{k+1}=\overline{\C} x_{k+1} + \overline{\D} u_k 
\end{cases}
\end{equation}
Crucially, the above system allows us to predict the value of the future input state $\widehat{u}_{k+1}$ based on the hidden state at $x_{k+1}$ and the input $u_k$, and hence perform autoregressive ICL.\par

\textbf{(3)} To further investigate the proposed parametrization above, we provide an asymptotic bound on the error incurred when approximating $\dot{u}(t)$ through a hidden state of finite dimension $N$, denoted by $\dot{u}_N(t)$. For this, we consider an alternative construction of the FouT basis, simplifying the analysis. Derivations of Prop. \ref{fout_altern} and Thm. \ref{local_approx_error} along with a Corollary for the error of signal predictions in the continuous setting are in Appendix \ref{App: Fout}.
\vspace{-2mm}
\begin{restatable}[Alternative FouT construction]{prop}{FouTAlt}
\label{fout_altern}
If we choose $\C_k = \begin{cases}
        0 & \text{if} \: k=0 \text{ or } k \text{ odd}\\
        -2 \sqrt{2}\pi n & \text{otherwise} \quad
    \end{cases}$,\\ $
    \D = 0$ and $\A$, $\B$ and $p_k(t,s)$ as in HiPPO FouT and if $u(t)$ has $k$-th bounded derivatives for some $k \geq 3$, then the output $y(t)$ is an approximation of $\dot{u}(t)$ based on $N$ basis functions.
\end{restatable}

\begin{restatable}[Approximation Error]{thm}{ApproxErr}
\label{local_approx_error}
    If $u$ has $k$-th bounded derivatives for some $k \geq 3$, then it holds that for the choice of $\A$ and $\B$ in Hippo FouT and $\C$ and $\D$ as in Prop. \ref{fout_altern}: $\left|\dot{u}(t) - \dot{u}_N(t)\right| \in \mathcal{O}(L/N^{k-2})$
\end{restatable}
%Thus we arrive at our discretized constructions $\overline{\C},\overline{\D}$, which result in a system that for $N\rightarrow \infty$ predicts the next value of the signal $u$ using first-order approximation.

%\color{blue}
%This section is a mixture of preliminaries, problem formulation and contains already the explicit weight construction for A and B
%\begin{itemize}
    %\item Preliminiaries covered: SSMs, HiPPO theory, LegS, LegT, FouT. 
   % \item Problem formulation: Dynamical system formulation.
    %\item Present the propositions for the explicit weight construction ($\C$, $\D$)
    %\item In the main text, we can also give the equations for the discretization $\overline{\C}, \overline{\D}$
%\end{itemize}
%\color{black}

==> sections_submission_old/problem_formulation_backup.tex <==
\section{Solving Dynamical Systems with SSMs}

State space models (SSM) take the following form:

\begin{equation}
    \begin{cases}
        \dot{x}(t) = \A x(t)+\B u(t) \\
        y(t) = \C x(t)+\D u(t)
    \end{cases}
\end{equation}

In our setting, we consider $u(t) \in \mathbb{R}$ and $x(t) \in \mathbb{R}^N$. Our paper builds on the HiPPo theory, a framework developed in \citep{NEURIPS2020_102f0bb6} and \citep{gu2022train}. This method provides specific parametrizations of the matrices $\A$ and $\B$ such that the hidden state $x(t)$ can be seen to represent an orthogonal projection of the input signal $u_{\leq t}$ onto the $N$-dimensional space of Lagrange polynomials or Fourier basis (or more in general of any complete orthogonal basis). In particular, the HiPPO theory considers an Hilbert space with orthogonal basis functions $\{ p_n(t,s)\}_{n \geq 0}$ and a measure $\omega(t,s)$, equipped with an inner product $\langle f, g \rangle_\omega = \int_{-\infty}^t f(s)g(s) \omega(t,s) ds$. Then, the goal is to construct $A$ and $B$ such that $x_n(t) = \int_{-\infty}^t u(s) p_n(t,s) \omega(t, s) ds$, i.e. $x_n(t)$ represents the projection of $u(s)$ on the basis $p_n(t,s)$ under the inner product of the space we are considering. We are going to review three of the methods proposed by HiPPO theory, their choice of basis and their respective constructions of $\A$ and $\B$ later in this section. The key takeaway of this approach is that $x(t)$ is storing all the information about the input signal up to time $t$.In particular, in the limit of $N \rightarrow \infty $ we have that:

\begin{equation}
\label{reconstruction}
    u(s) = \sum_{n=0}^{\infty} x_n(t) p_n(t,s) \ \ \forall s\leq t
\end{equation}

with $p_n(t,s)$ being the orthonormal basis. This means that in the limit of infinite hidden states dimension we can exactly recover the input signal at any time $s\leq t$ by only looking at the values of the hidden states at time $t$. Equivalently, this means that $x(t)$ serves as a memory of all the information contained in the input signal up to time $t$. The original goal  of this framework was indeed to show that it is possible to (approximately) recover the input signal up to the current time step by only having access to the current values of the hidden state. In this work however we plan to extend this framework in order to be able not only to recover the past input signals but also to predict the next input signal.\\
\\
HiPPO theory provides many different constructions for the matrices $\A$ and $\B$, but here we will focus on three of them in particular, namely HiPPO-LegT, HiPPO-LegS and HiPPO-FouT. The first two of them rely on projections on the space of Legendre polynomials, the first leading to a LTI system whereas the second leads to a time-varying system. The latter instead leverages projections on the space of Fourier basis, made of classical sine and cosine basis functions. 
\\
As mentioned above, the main goal of HiPPo theory is to construct matrices $A$ and $B$ to show that $x(t)$ is able to retain all the information about the input signal up until that point and only based on this information we can approximately reconstruct the signal until time $t$. However, this approach only focused on $A$, $B$ and $x(t)$ but never really considered $C$, $D$ and $y(t)$. In our work, we aim to leverage these to predict the value of the input at the next time step. More precisely, our goal will be, for each of the three aforementioned constructions of HiPPO Theory, to find a parametrization of $\C$ and $\D$ such that the output $y(t)$ corresponds to $\dot{u}(t)$ (in the limit of $N \rightarrow \infty)$. Note that once we have this equivalence, we can discretize the equation $\dot{u}(t) \approx y(t)=\C x(t)+\D u(t)$ in order to get an approximation of the next input.
\\
Note that \citep{gu2022train} and \citep{NEURIPS2020_102f0bb6} analyze the HiPPO theory in the continuous setting of SSMs as in this case it is more natural to construct Hilbert spaces with inner products and their parametrizations for $\A$ and $\B$. Only after they derived these parametrizations they discretize the system so that we can leverage this approach in practice as well. We will follow a similar approach: we will first derive the parametrization for $\C$ and $\D$ in the continuous setting as this has analytical and theoretical advantages and then we will derive their discretized versions that we will use in our experiments. We will now go on to show how to construct $\C$ and $\D$ for LegT, LegS and FouT.
\\
Starting from Equation \ref{reconstruction} and evaluate it at time $t$, we get that:

\begin{equation}
    \label{u_t_rec}
    u(t) = \sum_{n=0}^{\infty} x_n(t) p_n(t,t) 
\end{equation}

 
In order to get an expression for $\dot{u}(t)$, we start from Equation \ref{u_t_rec} and differentiate $u(t)$ by differentiating the series term by term. In order to so, we will assume for now that $u(t)$ satisfies the smoothness assumptions required to exchange series and derivative, e.g. \color{red} TODO: write smoothness assumptions on u \color{black}.Note that also in all the three constructions $p_n(t,t)$ is a constant w.r.t $t$. Then, we have the following:

\begin{equation}
\label{u_t_dec}
    \dot{u}(t) = \sum_{n=0}^{\infty} \dot{x}_n(t) p_n(t,t) 
\end{equation}

Starting from Equation \ref{u_t_dec}, we will construct the matrices $C$ and $D$ for the three methods. We will separate the two cases and we will first review the differences in these two methods, e.g. which basis and measure they assume and their different parametrizations of $\A$ and $\B$.

\subsection{HiPPo-LegT}

\begin{restatable}[LegT construction]{prop}{LegT}
    \label{prop:LegT}
    If we choose $\C_j = \sum_{k = 0}^N\A_{kj}p_k(t, t)$ and $
    \D = \sum_{k = 0}^N \B_k p_k(t, t)$ and $\A$, $\B$ and $p_k(t,t)$ as in HiPPO LegT, then the output $y(t)$ is an approximation of $\dot{u}(t)$ based on $N$ basis functions.
\end{restatable}

\vspace{3mm}

\subsection{HiPPo-LegS}


Then, the following result holds for $\C$ and $\D$
\begin{restatable}[LegS construction]{prop}{LegS}
    \label{prop:LegS}
    If we choose $\C_j = \sum_{k = 0}^N\frac{1}{t}\A_{kj}p_k(t, t)$ and $
    \D = \sum_{k = 0}^N \frac{1}{t}\B_k p_k(t, t)$ and $\A$, $\B$ and $p_k(t,t)$ as in HiPPO LegS, then the output $y(t)$ is an approximation of $\dot{u}(t)$ based on $N$ basis functions.
\end{restatable}
\vspace{3mm}

\subsection{HiPPO-FouT}


We now have the following result for construction of $\C$ and $\D$ for FouT:

\begin{restatable}[FouT construction]{prop}{FouT}
\label{fout}
If we choose $\C_j = \sum_{k = 0}^N\A_{kj}p_k(t, t)$ and $
    \D = \sum_{k = 0}^N \B_k p_k(t, t)$ and $\A$, $\B$ and $p_k(t,t)$ as in HiPPO FouT, then the output $y(t)$ is an approximation of $\dot{u}(t)$ based on $N$ basis functions.
\end{restatable}

\vspace{3mm}
\subsection{Discretization}
Note that to predict the next time-step $u(t+\Delta t)$, we need to approximate the following integral, having access to $u(t)$:
\begin{equation}
    u(t+\Delta t) = u(t) +\int_{t}^{t+\Delta t}\dot{u}(s) ds
\end{equation}

Since we cannot solve the integral in closed form, we will use discretization, and in particular, the bilinear (also called trapezoid) method. Note that we could use any other discretization methods (e.g. Forward/Backward Euler or Generalized Bilinear Transformation), but here we stick with the choice of the Bilinear method which is the most common one and exhibits nice stability properties. The Bilinear method leads to the following approximation (more details in the Appendix): \color{red} TODO: change into index notation instead of time notation \color{black}

\begin{align}
    u(t+ \Delta t) 
    &\approx \left( 1 - \frac{\D \Delta t}{2}\right)^{-1} \left[ \left( 1 + \frac{\D \Delta t}{2}\right)u(t) + \Delta t \C x(t) \right]\\
    &= \overline{\C} x(t)+ \overline{\D} u(t)
\end{align}

where $\C$ and $\D$ are the parametrizations of HiPPo LegT, LegS or FouT.

\vspace{1mm}

%\color{blue}
%This section is a mixture of preliminaries, problem formulation and contains already the explicit weight construction for A and B
%\begin{itemize}
    %\item Preliminiaries covered: SSMs, HiPPO theory, LegS, LegT, FouT. 
   % \item Problem formulation: Dynamical system formulation.
    %\item Present the propositions for the explicit weight construction ($\C$, $\D$)
    %\item In the main text, we can also give the equations for the discretization $\overline{\C}, \overline{\D}$
%\end{itemize}
%\color{black}

==> sections_submission_old/problem_formulation_backup_old.tex <==
\section{Solving Dynamical Systems with SSMs}
State space models (SSM) take the following form:
\begin{equation}
    \begin{cases}
        \dot{x}(t) = \A x(t)+\B u(t) \\
        y(t) = \C x(t)+\D u(t)
    \end{cases}
\end{equation}
In our setting, we consider $u(t) \in \mathbb{R}$ and $x(t) \in \mathbb{R}^N$. Our paper builds on the HiPPo theory, a framework developed in \citep{NEURIPS2020_102f0bb6} and \citep{gu2022train}. This method provides specific parametrizations of the matrices $\A$ and $\B$ such that the hidden state $x(t)$ can be seen to represent an orthogonal projection of the input signal $u_{\leq t}$ onto the $N$-dimensional space of Lagrange polynomials or Fourier basis (or more in general of any complete orthogonal basis). In particular, the HiPPO theory considers an Hilbert space with orthogonal basis functions $\{ p_n(t,s)\}_{n \geq 0}$ and a measure $\omega(t,s)$, equipped with an inner product $\langle f, g \rangle_\omega = \int_{-\infty}^t f(s)g(s) \omega(t,s) ds$. Then, the goal is to construct $A$ and $B$ such that $x_n(t) = \int_{-\infty}^t u(s) p_n(t,s) \omega(t, s) ds$, i.e. $x_n(t)$ represents the projection of $u(s)$ on the basis $p_n(t,s)$ under the inner product of the space we are considering. We are going to review three of the methods proposed by HiPPO theory, their choice of basis and their respective constructions of $\A$ and $\B$ later in this section. The key takeaway of this approach is that $x(t)$ is storing all the information about the input signal up to time $t$.In particular, in the limit of $N \rightarrow \infty $ we have that:
\begin{equation}
\label{reconstruction}
    u(s) = \sum_{n=0}^{\infty} x_n(t) p_n(t,s) \ \ \forall s\leq t
\end{equation}
with $p_n(t,s)$ being the orthonormal basis. This means that in the limit of infinite hidden states dimension we can exactly recover the input signal at any time $s\leq t$ by only looking at the values of the hidden states at time $t$. Equivalently, this means that $x(t)$ serves as a memory of all the information contained in the input signal up to time $t$. The original goal  of this framework was indeed to show that it is possible to (approximately) recover the input signal up to the current time step by only having access to the current values of the hidden state. In this work however we plan to extend this framework in order to be able not only to recover the past input signals but also to predict the next input signal.\\
\\
HiPPO theory provides many different constructions for the matrices $\A$ and $\B$, but here we will focus on three of them in particular, namely HiPPO-LegT, HiPPO-LegS and HiPPO-FouT. The first two of them rely on projections on the space of Legendre polynomials, the first leading to a LTI system whereas the second leads to a time-varying system. The latter instead leverages projections on the space of Fourier basis, made of classical sine and cosine basis functions. 
\\
As mentioned above, the main goal of HiPPo theory is to construct matrices $A$ and $B$ to show that $x(t)$ is able to retain all the information about the input signal up until that point and only based on this information we can approximately reconstruct the signal until time $t$. However, this approach only focused on $A$, $B$ and $x(t)$ but never really considered $C$, $D$ and $y(t)$. In our work, we aim to leverage these to predict the value of the input at the next time step. More precisely, our goal will be, for each of the three aforementioned constructions of HiPPO Theory, to find a parametrization of $\C$ and $\D$ such that the output $y(t)$ corresponds to $\dot{u}(t)$ (in the limit of $N \rightarrow \infty)$. Note that once we have this equivalence, we can discretize the equation $\dot{u}(t) \approx y(t)=\C x(t)+\D u(t)$ in order to get an approximation of the next input.
\\
Note that \citep{gu2022train} and \citep{NEURIPS2020_102f0bb6} analyze the HiPPO theory in the continuous setting of SSMs as in this case it is more natural to construct Hilbert spaces with inner products and their parametrizations for $\A$ and $\B$. Only after they derived these parametrizations they discretize the system so that we can leverage this approach in practice as well. We will follow a similar approach: we will first derive the parametrization for $\C$ and $\D$ in the continuous setting as this has analytical and theoretical advantages and then we will derive their discretized versions that we will use in our experiments. We will now go on to show how to construct $\C$ and $\D$ for LegT, LegS and FouT.
\\
Starting from Equation \ref{reconstruction} and evaluate it at time $t$, we get that:

\begin{equation}
    \label{u_t_rec}
    u(t) = \sum_{n=0}^{\infty} x_n(t) p_n(t,t) 
\end{equation}

 
In order to get an expression for $\dot{u}(t)$, we start from Equation \ref{u_t_rec} and differentiate $u(t)$ by differentiating the series term by term. In order to so, we will assume for now that $u(t)$ satisfies the smoothness assumptions required to exchange series and derivative, e.g. \color{red} TODO: write smoothness assumptions on u \color{black}.Note that also in all the three constructions $p_n(t,t)$ is a constant w.r.t $t$. Then, we have the following:

\begin{equation}
\label{u_t_dec}
    \dot{u}(t) = \sum_{n=0}^{\infty} \dot{x}_n(t) p_n(t,t) 
\end{equation}

Starting from Equation \ref{u_t_dec}, we will construct the matrices $C$ and $D$ for the three methods. We will separate the two cases and we will first review the differences in these two methods, e.g. which basis and measure they assume and their different parametrizations of $\A$ and $\B$.

\subsection{HiPPo-LegT}

\begin{restatable}[LegT construction]{prop}{LegT}
    \label{prop:LegT}
    If we choose $\C_j = \sum_{k = 0}^N\A_{kj}p_k(t, t)$ and $
    \D = \sum_{k = 0}^N \B_k p_k(t, t)$ and $\A$, $\B$ and $p_k(t,t)$ as in HiPPO LegT, then the output $y(t)$ is an approximation of $\dot{u}(t)$ based on $N$ basis functions.
\end{restatable}

\vspace{3mm}

\subsection{HiPPo-LegS}


Then, the following result holds for $\C$ and $\D$
\begin{restatable}[LegS construction]{prop}{LegS}
    \label{prop:LegS}
    If we choose $\C_j = \sum_{k = 0}^N\frac{1}{t}\A_{kj}p_k(t, t)$ and $
    \D = \sum_{k = 0}^N \frac{1}{t}\B_k p_k(t, t)$ and $\A$, $\B$ and $p_k(t,t)$ as in HiPPO LegS, then the output $y(t)$ is an approximation of $\dot{u}(t)$ based on $N$ basis functions.
\end{restatable}
\vspace{3mm}

\subsection{HiPPO-FouT}


We now have the following result for construction of $\C$ and $\D$ for FouT:

\begin{restatable}[FouT construction]{prop}{FouT}
\label{fout}
If we choose $\C_j = \sum_{k = 0}^N\A_{kj}p_k(t, t)$ and $
    \D = \sum_{k = 0}^N \B_k p_k(t, t)$ and $\A$, $\B$ and $p_k(t,t)$ as in HiPPO FouT, then the output $y(t)$ is an approximation of $\dot{u}(t)$ based on $N$ basis functions.
\end{restatable}

\vspace{3mm}
\subsection{Discretization}
Note that to predict the next time-step $u(t+\Delta t)$, we need to approximate the following integral, having access to $u(t)$:
\begin{equation}
    u(t+\Delta t) = u(t) +\int_{t}^{t+\Delta t}\dot{u}(s) ds
\end{equation}

Since we cannot solve the integral in closed form, we will use discretization, and in particular, the bilinear (also called trapezoid) method. Note that we could use any other discretization methods (e.g. Forward/Backward Euler or Generalized Bilinear Transformation), but here we stick with the choice of the Bilinear method which is the most common one and exhibits nice stability properties. The Bilinear method leads to the following approximation (more details in the Appendix): \color{red} TODO: change into index notation instead of time notation \color{black}

\begin{align}
    u(t+ \Delta t) 
    &\approx \left( 1 - \frac{\D \Delta t}{2}\right)^{-1} \left[ \left( 1 + \frac{\D \Delta t}{2}\right)u(t) + \Delta t \C x(t) \right]\\
    &= \overline{\C} x(t)+ \overline{\D} u(t)
\end{align}

where $\C$ and $\D$ are the parametrizations of HiPPo LegT, LegS or FouT.

\vspace{1mm}

%\color{blue}
%This section is a mixture of preliminaries, problem formulation and contains already the explicit weight construction for A and B
%\begin{itemize}
    %\item Preliminiaries covered: SSMs, HiPPO theory, LegS, LegT, FouT. 
   % \item Problem formulation: Dynamical system formulation.
    %\item Present the propositions for the explicit weight construction ($\C$, $\D$)
    %\item In the main text, we can also give the equations for the discretization $\overline{\C}, \overline{\D}$
%\end{itemize}
%\color{black}

==> sections_submission_old/some_old.tex <==
%\section{Main}
%State space models (SSM) take the following form:

%\begin{equation}
    %\begin{cases}
        %\dot{x}(t) = \A x(t)+\B u(t) \\
        %y(t) = \C x(t)+\D u(t)
    %\end{cases}
%\end{equation}

%In our setting, we consider $u(t) \in \mathbb{R}$ and $x(t) \in \mathbb{R}^N$. It was proven in \citep{NEURIPS2020_102f0bb6} and \citep{gu2022train} that by choosing the matrices $\A$ and $\B$ according to the HIPPO theory, then the hidden state $x(t)$ can be seen to represent an orthogonal projection of the input signal $u_{\leq t}$ onto the $N$-dimensional space of Lagrange polynomials. In particular, in the limit of $N \rightarrow \infty $ we have that:

%\begin{equation}
    %u(s) = \sum_{n=0}^{\infty} x_n(t) p_n(t,s) \ \ \forall s\leq t
%\end{equation}

%with $p_n(t,s)$ being the orthonormal basis. In particular, they consider two settings, namely Hippo-LegT and Hippo-LegS, based on Legendre polynomials, but the first leads to a time-invariant LTI, whereas the second leads to a time-variant system. From above, we easily get that:

%\begin{equation}
%\label{u_t_decomp}
    %u(t) = \sum_{n=0}^{\infty} x_n(t) p_n(t,t) 
%\end{equation}

%The idea behind this construction in \citep{NEURIPS2020_102f0bb6} and \citep{gu2022train} is that $x(t)$ can (approximately) retain all the information up until time $t$ and hence we can approximately reconstruct the input signal up until the current time by using $x(t)$. In this work, we want to take this construction a step further, and in particular, we want to leverage the HiPPO theory to also approximate any first-order dynamical system. In particular, we will show how to construct a parametrization of $\C$ and $\D$ such that $y(t)=\dot{u}(t)$ (in the limit of $N \rightarrow \infty$). 
%To do so, we start from Equation \ref{u_t_decomp} and differentiate $u(t)$ by differentiating the series term by term. We will assume for now that $u(t)$ satisfies the smoothness assumptions required to exchange series and derivative, and we will specify the specific assumptions that $u(t)$ needs to satisfy later. \color{red} TODO: write down formal assumptions in the Propositions\color{black}. Note that also in both LegT and LegS $p_n(t,t)$ is a constant \color{red} TODO: maybe write down explicitly what $p_n(t,s)$ looks like in the two cases \color{black}. Then, we have the following:

%\begin{equation}
%\label{u_t_decomp}
    %\dot{u}(t) = \sum_{n=0}^{\infty} \dot{x}_n(t) p_n(t,t) 
%\end{equation}

%We will now derive the parametrizations for $\C$ and $\D$ for both LegT and LegS, starting from the above equation. We have the following two results:
%\begin{restatable}[LegT construction]{prop}{LegT}
    %\label{prop:LegT}
    %If we choose $\C_j = \sum_{k = 0}^N\A_{kj}p_k(t, t)$ and $
    %\D = \sum_{k = 0}^N \B_k p_k(t, t)$ and $\A$, $\B$ and $p_k(t,t)$ as in HiPPO LegT, then the output $y(t)$ is an $N$-dimensional approximation of $\dot{u}(t)$.
%\end{restatable}
%\vspace{-0.3cm}
%\begin{restatable}[LegS construction]{prop}{LegS}
    %\label{prop:LegS}
    %If we choose $\C_j = \sum_{k = 0}^N\frac{1}{t}\A_{kj}p_k(t, t)$ and $
    %\D = \sum_{k = 0}^N \frac{1}{t}\B_k p_k(t, t)$ and $\A$, $\B$ and $p_k(t,t)$ as in HiPPO LegS, then the output $y(t)$ is an $N$-dimensional approximation of $\dot{u}(t)$.
%\end{restatable}
%Note that to predict the next time-step $u(t+\Delta t)$, we need to approximate the following integral, having access to $u(t)$:
%\begin{equation}
    %u(t+\Delta t) = u(t) +\int_{t}^{t+\Delta t}\dot{u}(s) ds
%\end{equation}

%Since we cannot solve the integral in closed form, we will use discretization, and in particular, the bilinear (also called trapezoid) method, which leads to the following approximation (more details in the Appendix): \color{red} TODO: change into index notation instead of time notation \color{black}

%\begin{align}
    %u(t+ \Delta t) 
    %&\approx \left( 1 - \frac{\D \Delta t}{2}\right)^{-1} \left[ \left( 1 + \frac{\D \Delta t}{2}\right)u(t) + \Delta t \C x(t) \right]\\
   % &= \overline{\C} x(t)+ \overline{\D} u(t)
%\end{align}

%where $C$ and $D$ are the parametrizations of HiPPo LegT and LegS (the discretization leads to the same expression for both methods).\\

%We now propose a different way to calculate $\dot{u}(t)$, which we will base our theoretical analysis on. In particular, instead of first evaluating $u(s)$ at $t$ and then taking the derivative, we will first derive $u(s)$ and only then evaluate the function at $t$. The other difference is that here, we will use the classic Fourier basis of sines and cosines to make the analysis easier. In particular, we have the following:

%\begin{equation}
    %\dot{u}(s) = \sum_{n=0}^{\infty} x_n(t) \frac{\partial}{\partial s}p_n(t,s) \ \ \forall s < t
%\end{equation}

%Note that by assuming continuity of $\dot{u}$ and $p_n$ wrt $s$, we can take the limit from the left as $s$ goes to $t$, giving us:

%\begin{equation}
    %\dot{u}(t) = \sum_{n=0}^{\infty} x_n(t) \frac{\partial}{\partial s}p_n(t,s) \Big |_{s=t} 
%\end{equation}

%HiPPo-FouT assumes $\{p_n\}_{n \geq 0}(t,s) = \sqrt{2} \Big [1 \ \cos(2\pi (t-s)) \ \sin(2\pi (t-s)) \ \cos(4\pi (t-s)) \ \sin(4\pi (t-s)) \ \dots \Big]$ and $\omega(s,t)= \mathbb{1}_{[t-1, t]}(s)$. We now have the following construction of $\C$ and $\D$ for the Fourier basis.

%\begin{restatable}[FouT construction]{prop}{FouT}
%\label{fout}
%If we choose $\C_k = \begin{cases}
        %0 & \text{if} \: k=0 \text{ or } k \text{ odd}\\
       % -2\sqrt{2}\pi n & \text{otherwise} \quad
    %\end{cases}$ \ \ \ and $
    %\D = 0$ and $\A$, $\B$ and $p_k(t,s)$ as in HiPPO FouT, then the output $y(t)$ is an $N$-dimensional approximation of $\dot{u}(t)$.
%\end{restatable}

%In this case, note that we then have $\dot{u}(t) = Cx(t)$. For discretization, we will here use the simpler Euler method instead as it proves sufficiently stable for our purposes:

%\begin{equation}
    %u(t+\Delta t)-u(t) = \int_t^{t+\Delta t} \dot{u}(s) ds \approx \Delta t \dot{u}(t) = \Delta t C x(t)
%\end{equation}

%Hence we have $u(t+\Delta t) = \Delta t C x(t) + u(t)$, which leads to the choice $\overline{C} = \Delta t \ C$ and $\overline{D} = 1$.

%\subsection{Theoretical Analysis}

%Given the above construction, we now want to find a bound on the approximation error that we make by truncating the expansion of $\dot{u}(t)$ up to N terms. We will denote this approximation $\dot{u}_N(t)$. From this, We will also derive an approximation bound on $\widehat{u}_N(t)$, where $\widehat{u}_N(t) = \int_{0}^t \dot{u}_N(s) ds$ is the approximation of $u(t)$ by integrating the truncated version of its time derivative. This reflects the way we derive an estimate of the next step of $u$ in this work. Please note that we will not consider the error coming from the discretization in this work for simplicity of explanation and leave this to future work. Let us note that we will also focus on the FouT parametrization in this work. We will leave the analysis of LegT for future work. We have the following results:

%\begin{restatable}[Local Approximation Error]{thm}{ApproxErr}
%\label{approx_error}
    %If $u$ has k-th bounded derivatives with $k \geq 3$, i.e. $u^{(k)}(t) \leq L \ \forall t$, then it holds that for the choice of $\A$ and $\B$ in Hippo FouT and $\C$ and $\D$ as in Prop. \ref{fout}:

    %\begin{equation*}
        %\left|\dot{u}(t) - \dot{u}_N(t)\right| \in \mathcal{O}\left(\frac{L}{N^{k-2}}\right)
    %\end{equation*}
%\end{restatable}

%\begin{restatable}[Approximation Error]{thm}{ApproxErr}
%\label{approx_error}
    %If $u(t)$ is L-Lipschitz and twice differentiable and $\dot{u}(t)$ is M-Lipschitz, then the following holds for HiPPO LegS:
    %\begin{equation*}
    %\|\dot{u}(t) - \dot{u}_N(t)\|_2 \in \mathcal{O}\left(\sqrt{\frac{L^2 + LMt + M^2t}{N}}\right)
    %\end{equation*}
%\end{restatable}

%As a corollary of the above, we get that:

%\begin{restatable}[Approximation Error]{cor}{ApproxErrCor}
%\label{cor:ApproxErrCor}
    %Under the same assumptions and parametrization as in Theorem \ref{approx_error}, we have that:

     %\begin{equation*}
        % \left|u(t) - \widehat{u}_N(t)\right| \in \mathcal{O}\left(\frac{Lt}{N^{k-2}}\right)
      %\end{equation*}
    
%\end{restatable}

%\begin{restatable}[Approximation Error]{cor}{ApproxErrCor}
%\label{cor:ApproxErrCor}
    %Under the same assumption as in Theorem \ref{approx_error}, we have that for Hippo-LegS:
    %\begin{equation*}
       % \|u(t) - u_N(t)\|_2 
    %\in \mathcal{O}\left(t\sqrt{\frac{L^2 + LMt + t^2}{N}}\right)
    %\end{equation*}
%\end{restatable}

%As we expect, we have that the error decreases as N increases, i.e. as we consider more basis into the approximation and increases over time.\\
%For completeness, we will also report a global guarantee for the L2-error of $\dot{u}_N(s)$ and a fixed $t$. In particular, we have the following result:

%\begin{restatable}
    %[Global Approximation Error]{thm}{GlobalApproxErr}
    %If $u$ has k-th bounded derivatives with $k \geq 2$, then for the FouT parametrization it holds that:

    %\begin{equation*}
        %\|\dot{u} - \dot{u}_N\|_{2,\omega}^2 \in \mathcal{O}\left(\frac{L^2}{N^{2k-3}}{}\right)
    %\end{equation*}
    
%\end{restatable}



==> sections_submission_old/theoretical_analysis.tex <==
\section{Theoretical Analysis}

\color{red} TODO: Finish to incorporate Caglar's comments in this section \color{black}\\

Given the above construction, we now want to find a bound on the approximation error we make by truncating the expansion of $\dot{u}(t)$ up to N terms. We will denote this approximation $\dot{u}_N(t)$. From this, We will also derive an approximation bound on $\widehat{u}_N(t)$, where $\widehat{u}_N(t) = \int_{0}^t \dot{u}_N(s) ds$ is the approximation of $u(t)$ by integrating the truncated version of its time derivative. This reflects the way we derive an estimate of the next step of $u$ in this work. Please note that we will not consider the error coming from the discretization in this work for simplicity of explanation and leave this to future work. Let us note that we will also focus on the FouT parametrization in this work. We will leave the analysis of LegT for future work. We have the following results:

\begin{restatable}[Local Approximation Error]{thm}{ApproxErr}
\label{approx_error}
    If $u$ has k-th bounded derivatives for some $k \geq 3$, i.e. $|u^{(k)}(t)| \leq L \ \forall t$, then it holds that for the choice of $\A$ and $\B$ in Hippo FouT and $\C$ and $\D$ as in Prop. \ref{fout}:

    \begin{equation*}
        \left|\dot{u}(t) - \dot{u}_N(t)\right| \in \mathcal{O}\left(\frac{L}{N^{k-2}}\right)
    \end{equation*}
\end{restatable}

%\begin{restatable}[Approximation Error]{thm}{ApproxErr}
%\label{approx_error}
    %If $u(t)$ is L-Lipschitz and twice differentiable and $\dot{u}(t)$ is M-Lipschitz, then the following holds for HiPPO LegS:
    %\begin{equation*}
    %\|\dot{u}(t) - \dot{u}_N(t)\|_2 \in \mathcal{O}\left(\sqrt{\frac{L^2 + LMt + M^2t}{N}}\right)
    %\end{equation*}
%\end{restatable}

As a corollary of the above, we get that:

\begin{restatable}[Approximation Error]{cor}{ApproxErrCor}
\label{cor:ApproxErrCor}
    Under the same assumptions and parametrization as in Theorem \ref{approx_error}, we have that:

     \begin{equation*}
         \left|u(t) - \widehat{u}_N(t)\right| \in \mathcal{O}\left(\frac{Lt}{N^{k-2}}\right)
      \end{equation*}
    
\end{restatable}

%\begin{restatable}[Approximation Error]{cor}{ApproxErrCor}
%\label{cor:ApproxErrCor}
    %Under the same assumption as in Theorem \ref{approx_error}, we have that for Hippo-LegS:
    %\begin{equation*}
       % \|u(t) - u_N(t)\|_2 
    %\in \mathcal{O}\left(t\sqrt{\frac{L^2 + LMt + t^2}{N}}\right)
    %\end{equation*}
%\end{restatable}

As we expect, we have that the error decreases as N increases, i.e. as we consider more basis into the approximation and increases over time.\\
For completeness, we will also report a global guarantee for the L2-error of $\dot{u}_N(s)$ and a fixed $t$. In particular, we have the following result:

\begin{restatable}
    [Global Approximation Error]{thm}{GlobalApproxErr}
    If $u$ has k-th bounded derivatives for some $k \geq 2$, then for the FouT parametrization it holds that:

    \begin{equation*}
        \|\dot{u} - \dot{u}_N\|_{2,\omega}^2 \in \mathcal{O}\left(\frac{L^2}{N^{2k-3}}{}\right)
    \end{equation*}
    
\end{restatable}

==> sections_submission_old/theoretical_analysis_old.tex <==
\section{Theoretical Analysis}

Given the above construction, we now want to find a bound on the approximation error we make by truncating the expansion of $\dot{u}(t)$ up to N terms. We will denote this approximation $\dot{u}_N(t)$. From this, We will also derive an approximation bound on $\widehat{u}_N(t)$, where $\widehat{u}_N(t) = \int_{0}^t \dot{u}_N(s) ds$ is the approximation of $u(t)$ by integrating the truncated version of its time derivative. This reflects the way we derive an estimate of the next step of $u$ in this work. Please note that we will not consider the error coming from the discretization in this work for simplicity of explanation and leave this to future work. Let us note that we will also focus on the FouT parametrization in this work. We will leave the analysis of LegT for future work. We have the following results:

\begin{restatable}[Local Approximation Error]{thm}{ApproxErr}
\label{approx_error}
    If $u$ has k-th bounded derivatives for some $k \geq 3$, i.e. $|u^{(k)}(t)| \leq L \ \forall t$, then it holds that for the choice of $\A$ and $\B$ in Hippo FouT and $\C$ and $\D$ as in Prop. \ref{fout}:

    \begin{equation*}
        \left|\dot{u}(t) - \dot{u}_N(t)\right| \in \mathcal{O}\left(\frac{L}{N^{k-2}}\right)
    \end{equation*}
\end{restatable}

%\begin{restatable}[Approximation Error]{thm}{ApproxErr}
%\label{approx_error}
    %If $u(t)$ is L-Lipschitz and twice differentiable and $\dot{u}(t)$ is M-Lipschitz, then the following holds for HiPPO LegS:
    %\begin{equation*}
    %\|\dot{u}(t) - \dot{u}_N(t)\|_2 \in \mathcal{O}\left(\sqrt{\frac{L^2 + LMt + M^2t}{N}}\right)
    %\end{equation*}
%\end{restatable}

As a corollary of the above, we get that:

\begin{restatable}[Approximation Error]{cor}{ApproxErrCor}
\label{cor:ApproxErrCor}
    Under the same assumptions and parametrization as in Theorem \ref{approx_error}, we have that:

     \begin{equation*}
         \left|u(t) - \widehat{u}_N(t)\right| \in \mathcal{O}\left(\frac{Lt}{N^{k-2}}\right)
      \end{equation*}
    
\end{restatable}

%\begin{restatable}[Approximation Error]{cor}{ApproxErrCor}
%\label{cor:ApproxErrCor}
    %Under the same assumption as in Theorem \ref{approx_error}, we have that for Hippo-LegS:
    %\begin{equation*}
       % \|u(t) - u_N(t)\|_2 
    %\in \mathcal{O}\left(t\sqrt{\frac{L^2 + LMt + t^2}{N}}\right)
    %\end{equation*}
%\end{restatable}

As we expect, we have that the error decreases as N increases, i.e. as we consider more basis into the approximation and increases over time.\\
For completeness, we will also report a global guarantee for the L2-error of $\dot{u}_N(s)$ and a fixed $t$. In particular, we have the following result:

\begin{restatable}
    [Global Approximation Error]{thm}{GlobalApproxErr}
    If $u$ has k-th bounded derivatives for some $k \geq 2$, then for the FouT parametrization it holds that:

    \begin{equation*}
        \|\dot{u} - \dot{u}_N\|_{2,\omega}^2 \in \mathcal{O}\left(\frac{L^2}{N^{2k-3}}{}\right)
    \end{equation*}
    
\end{restatable}
